End-to-end Generative Pretraining for Multimodal Video Captioning

Recent video and language pretraining frameworks lack the ability to generate sentences. We present Multimodal Video Generative Pretraining (MV-GPT), a new pretraining framework for learning from unlabelled videos which can be effectively used for generative tasks such as multimodal video captioning. Unlike recent video-language pretraining frameworks, our framework trains both a multimodal video encoder and a sentence decoder jointly. To overcome the lack of captions in unlabelled videos, we leverage the future utterance as an additional text source and propose a bidirectional generation objective -- we generate future utterances given the present mulitmodal context, and also the present utterance given future observations. With this objective, we train an encoder-decoder model end-to-end to generate a caption from raw pixels and transcribed speech directly. Our model achieves state-of-the-art performance for multimodal video captioning on four standard benchmarks, as well as for other video understanding tasks such as VideoQA, video retrieval and action classification.

==> CVPR 2022 MV-GPT for final arXiv/sections/abstract.tex <==
\begin{abstract}
Recent video and language pretraining frameworks lack the ability to generate sentences.
We present Multimodal Video Generative Pretraining (MV-GPT), a new pretraining framework for learning from unlabelled videos which can be effectively used for generative tasks such as multimodal video captioning. 
Unlike recent video-language pretraining frameworks, our framework trains both a multimodal video encoder and a sentence decoder jointly.
To overcome the lack of captions in unlabelled videos, we leverage the future utterance as an additional text source and propose a bidirectional generation objective -- we generate future utterances given the present mulitmodal context, and also the present utterance given future observations.
With this objective, we train an encoder-decoder model end-to-end to generate a caption from raw pixels and transcribed speech directly.
Our model achieves state-of-the-art performance for multimodal video captioning on four standard benchmarks, as well as for other video understanding tasks such as VideoQA, video retrieval and action classification.

\end{abstract}


==> CVPR 2022 MV-GPT for final arXiv/sections/conclusion.tex <==
\section{Conclusion}
We present a novel generative pretraining framework for multimodal video captioning. Our bi-directional generative objective jointly trains an encoder for multimodal inputs and a decoder to generate meaningful captions, by using utterances sampled at different times in unlabelled videos. The model is trained end-to-end both during pretraining and finetuning, and achieves state-of-the-art results on multiple video captioning benchmarks as well as  on other video understanding tasks, namely VideoQA, video retrieval and action classification. 


%}

% \anurag{CVPR reviewers may not notice subtleties. So consider naming the paragraph ``Limitations'' or ``Broader impact'' and so on.}



==> CVPR 2022 MV-GPT for final arXiv/sections/experiments.tex <==
\section{Experiments}
In this section, we first demonstrate our results on four different benchmarks for multimodal video captioning. We then also show that our pretrained model has the ability to generalise to other video understanding tasks such as video question answering (VideoQA), video retrieval and action classification.

\subsection{Multimodal Video Captioning}
\label{sec:exp_captioning}


\subsubsection{Datasets and Evaluation Protocols}
We use HowTo100M~\cite{miech2019howto100m} as our pretraining dataset, and evaluate on four downstream captioning benchmarks. \\ %, described below.\\
\noindent\textbf{HowTo100M}~\cite{miech2019howto100m} consists of 1.2M instructional videos from YouTube. Transcribed speech is obtained using the YouTube ASR API~\cite{youtubeapi}.
Following \cite{seo2021look}, we extract 53M triplets of frames, current utterances and future utterances for pretraining.


\noindent\textbf{YouCook2}~\cite{zhou2018towards} is the most widely adopted benchmark for multimodal video captioning and contains 2,000 cooking videos for 89 different dishes with 14K video clips. 
Each video clip is annotated with a single captioning sentence.

\noindent\textbf{Video Timeline Tags (ViTT)}~\cite{huang2020multimodal} 
was created to better reflect the distribution of instructional videos in the wild. 
It consists of 8,169 videos, 5,840 of these videos for training and the remaining videos for validation and testing. 
Videos are divided into 7.1 segments on average, with each segment accompanied by a short timeline tag.

\noindent\textbf{MSR-VTT}~\cite{xu2016msr} is a standard benchmark with 10K open domain video clips for video captioning.
The duration of each video clip is between 10 and 30 seconds, and 20 natural language descriptions are manually annotated per clip.

\noindent\textbf{ActivityNet-Captions}~\cite{krishna2017dense} is a standard dense video captioning benchmark consisting of 100K temporally localized
sentences for 20k videos. 
We follow the standard splits with 50/25/25\% examples for training, validation and test sets.
To evaluate our model's ability to predict captions, we use ground truth temporal proposals following~\cite{krishna2017dense}.

We pretrain a single model on HowTo100M, which is then transferred to all four captioning benchmarks through finetuning. 
We report results using the following established metrics: BLEU-4 (B-4)~\cite{papineni2002bleu}, CIDEr (C)~\cite{vedantam2015cider}, METEOR (M)~\cite{banerjee2005meteor} and ROUGE-L (R-L)~\cite{lin2004rouge}. 
For ViTT, we measure BLEU-1 (B-1) instead of BLEU-4 following \cite{huang2020multimodal}.

\subsubsection{Results}
In this section we ablate some key design choices, in particular the backbone and objective functions used in MV-GPT, and explore the impact of the end-to-end training.
Finally, we compare our model to the state of the art.


\begin{table}[t]
    \centering
    \scalebox{0.85}{
     \begin{tabular}{@{\hskip 0.8mm}l@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 0.8mm}}
    \toprule
        PT Losses  & PT parts & B-4 & C & M & R-L \\
    \midrule 
 No PT & -- & 13.25 & 1.03 & 17.56 & 35.48 \\
 Baseline PT & E & 16.13 & 1.46 & 21.76 & 41.50 \\
 CoMVT~\cite{seo2021look} & E & 14.46 & 1.24 & 18.46 & 37.17 \\
 M-MASS~\cite{huang2020multimodal} & E+D & 19.03 & 1.88 & 24.00 & 45.10 \\
 UniVL~\cite{luo2020univl} & E+D & 19.95 & 1.98 & 25.27 & 46.81 \\
 MV-GPT (Ours) & E+D & \bf21.26 & \bf2.14 & \bf26.36 & \bf48.58 \\ 
    \bottomrule
    \end{tabular}}
    \caption{
    Comparisons to existing pretraining losses on YouCook2. 
    \textbf{PT} stands for pretraining. \textbf{PT parts} indicates which part of the model are pretrained, encoder (E) or both encoder and decoder (E + D).
    We reimplement the loss functions of existing methods but use our model and training strategies for fair comparison. 
    } 
    \label{tab:comps-loss}
\end{table}



\noindent\textbf{Pretraining Losses:} 
We implement a simple baseline, which consists of a masked language modelling loss given visual frames and ASR as input (Baseline PT). 
We also reimplement three state-of-the-art pretraining losses: (i)~CoMVT~\cite{seo2021look}, (ii)~UniVL~\cite{luo2020univl} and (iii)~M-MASS~\cite{huang2020multimodal}. For a fair comparison, we use our model architecture for all experiments, varying the loss function only. For the methods which pretrain the encoder only, we initialise the decoder with public GPT-2 weights~\cite{radford2019language}. 
For `No PT', the encoder is not pretrained either, but is initialized with public BERT and ViViT pretrained on ImageNet21k.

Table~\ref{tab:comps-loss} compares these different losses. We can observe that  pretraining the encoder only brings moderate gains over training from scratch, for all the losses investigated.
This performance is greatly improved by pretraining both the encoder and decoder jointly. Finally, we observe that our approach MV-GPT outperforms existing joint pretraining losses. 






\begin{table}[t]
    \centering
    \scalebox{0.85}{
     \begin{tabular}{@{\hskip 0.8mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 0.8mm}}
    \toprule
        FG & BG & MLM-E & MLM-D & WD & B-4 & C & M & R-L \\
    \midrule 
 \multicolumn{5}{c}{\textit{No PT}}& 13.25 & 1.03 & 17.56 & 35.48 \\
  & & \checkmark & & & 16.13 & 1.46 & 21.76 & 41.50 \\ % 908K
 \checkmark & & \checkmark & & & 20.65 & 2.05 & 25.81 & 47.22 \\ % 908K
 \checkmark & & & \checkmark & & 20.77 & 2.09 & 25.90 & 47.41 \\
 \checkmark & \checkmark & \checkmark & & & 20.82 & 2.10 & 26.20 & 48.22 \\ % 1370K
 \checkmark & \checkmark & & \checkmark & &  20.89 & 2.11 & 26.42 & 48.30 \\ 
 \checkmark & \checkmark & & \checkmark & \checkmark & \bf21.26 & \bf2.14 & \bf26.36 & \bf48.58 \\ 
    \bottomrule
    \end{tabular}}
    \caption{Ablation on YouCook2 showing the effect of our different loss components in pretraining. \textbf{FG:} Forward Generation loss. \textbf{BG:} Backward Generation loss. \textbf{MLM-E/MLM-D:} Masked Language Modelling loss applied on encoder outputs (E) or decoder outputs (D). \textbf{WD:} Weight Decay. \textbf{No PT:} No pretraining with any of these losses.
    } 
    \label{tab:abl-losses}
\end{table}
\noindent\textbf{Effect of each Loss Term in MV-GPT:}
Table~\ref{tab:abl-losses} shows the effect of each term in our loss function. 
The forward generation (FG) loss already provides strong supervision.
When applying the masked language modelling loss on the decoder outputs (MLM-D) instead of the encoder outputs (MLM-E), performance is slightly improved due to the additional input contextualization provided by the decoder.
Adding the backward generation (BG) loss provides a boost across all metrics.  
Additionally, we observe that adding weight decay (WD)~\cite{krogh1992simple} brings additional gains, and we report our scores in this full setting for the rest of the paper.


\begin{table}[t]
    \centering
    \scalebox{0.76}{
    \begin{tabular}{@{\hskip 0.8mm}c@{\hskip 1.5mm}c@{\hskip 3mm}c@{\hskip 2mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 0.8mm}}
    \toprule
        \multirow{2}{*}{Arch.}  & \multirow{2}{*}{Weights from / Trained on} & \multicolumn{2}{@{\hskip 0mm}c@{\hskip 3mm}}{E2E} & \multirow{2}{*}{B-4} & \multirow{2}{*}{C} & \multirow{2}{*}{M} & \multirow{2}{*}{R-L} \\
        &&PT&FT\\
    \midrule 
    \multicolumn{8}{c}{\textit{YouCook2}} \\
    \midrule
S3D & S3D \cite{xie2018rethinking} / Kinetics & & & 19.65 & 1.93 & 24.47 & 45.79 \\% 1254K
S3D & MIL-NCE \cite{miech2020end} / HowTo100M & & & 20.02 & 1.96 & 24.98 & 46.65 \\ % 1268K
 \hdashline
ViViT & ViViT \cite{arnab2021vivit} / Kinetics & & & 19.54 & 1.93 & 24.42 & 45.93 \\
ViViT & MV-GPT / HowTo100M & \checkmark & & 21.77 & 2.20 & 26.97 & 49.29 \\
ViViT & MV-GPT / HowTo100M & \checkmark & \checkmark & 21.26 & 2.14 & 26.36 & 48.58 \\
ViViT & MV-GPT / HowTo100M & \checkmark & \checkmark$\dagger$ & \bf21.88 & \bf2.21 & \bf27.09 & \bf49.38 \\
    \midrule
    \multicolumn{8}{c}{\textit{MSR-VTT}} \\
    \midrule
ViViT & MV-GPT / HowTo100M & \checkmark & & 47.04 & 0.55 & 36.80 & 62.99 \\
ViViT & MV-GPT / HowTo100M & \checkmark & \checkmark & \bf48.92 & \bf0.60 & \bf38.66 & \bf64.00 \\
    \bottomrule
    \end{tabular}}
    \caption{Ablation on YouCook2 with different visual encoder configurations.
    \textbf{E2E:} End-to-end training including the visual encoder.
    \textbf{PT:} Pretraining.
    \textbf{FT:} Finetuning.
    $\dagger$~Freeze the visual encoder at the beginning and tune end-to-end once converged during finetuning.
    }
    \label{tab:abl-backbone}
\vspace{-0.3cm}
\end{table}


\noindent\textbf{Visual Encoder and End-to-end Training:}
In Table~\ref{tab:abl-backbone}, we first compare the ViViT~\cite{arnab2021vivit} encoder to commonly used S3D features~\cite{xie2018rethinking}.
When both encoders are trained on Kinetics and fixed for multimodal pretraining and finetuning, they show comparable scores despite the large complexity of S3D due to the high frame rate required (30 fps vs.\ 1 fps for ViViT).
Using HowTo100M to train a visual encoder, we observe large gains with both architectures as expected given the similarity in the domains -- HowTo100M and YouCook2 are both instructional video datasets.
However, we observe larger gains with ViViT where the visual encoder is optimized for  generative losses within our framework and jointly trained with the other components thanks to the low complexity of the ViViT encoder. 
%\arsha{What is the low complexity referring to here?}
These results show the benefits of end-to-end pretraining.


We further investigate the effects of end-to-end training for finetuning. 
For YouCook2, we observe slight performance degradation when naively finetuning the network end-to-end from the beginning (row 4 to 5).
This degradation is overcome by initially freezing the visual encoder and starting end-to-end training after convergence, which gives us a minor gain (row 6).
These results indicate that our pretrained visual encoder already captures strong representations for inputs in a similar domain, and end-to-end finetuning is less critical in this case.
However, we observe more significant gains on MSR-VTT since end-to-end finetuning becomes crucial given a larger domain gap (row 7 to 8).

\begin{table}[t]

\vspace{-0.1cm}
    \centering
    \scalebox{0.85}{
    \begin{tabular}{@{\hskip 0.8mm}cc@{\hskip 2mm}c@{\hskip 2mm}c@{\hskip 2mm}c@{\hskip 2mm}c@{\hskip 0.8mm}}
    \toprule
    Initialization & MV-GPT Pretraining & B-4 & C & M & R-L \\ 
    \midrule 
        Random & & 10.93 & 64.56 & 12.88 & 29.03  \\
        Random &$\checkmark$ & 20.78 & 2.09 & 25.83 & 47.76   \\
        Public weights & & 13.25 & 1.03 & 17.56 & 35.48\\
        Public weights &$\checkmark$ & \bf21.26 & \bf2.14 & \bf26.36 & \bf48.58   \\
        % RandInit & 8.46  & 0.22 & 8.14 & 23.03  \\
        % BERT+GPT+ViViT & 12.49 & 0.93 & 16.07 & 34.00\\
        % MV-GPT & 19.04 & 1.86 & 24.04 & 45.22   \\
    \bottomrule
    \end{tabular}}
    \caption{Ablations on YouCook2 showing the effect of initialization and pretraining. \textbf{Public Weights}: Initialization with public BERT, GPT-2 and ViViT weights.
    % \textbf{MV-GPT}: Pretraining with our method.
    } 
    \label{tab:scratch}
\end{table}

\noindent\textbf{Pretraining with Random Initialization:}
We also investigate the ability of the model to learn from scratch.
We initialize the model either entirely randomly or using pretrained BERT, ViViT and GPT-2 weights.
Table~\ref{tab:scratch} shows that with random initialization, our method still performs very well (row 2), outperforming the model initalized with public BERT, GPT-2 and ViViT weights (row 3). Note that the pretrained ViViT weights were obtained from training on the fully supervised dataset Kinetics. 
Also, pretraining entirely from scratch even approaches the case where all parts of the model are intialized using public weights and pretrained (row 4).

\noindent\textbf{Multimodal vs.\ Single Modality:}
In Table~\ref{tab:sota-youcook}, we show results with text only and visual only inputs (we only feed the \texttt{CLS} token for the omitted modality). It is clear that both modalities are complementary and performance is best when combining both.
Additionally, to assess the contribution of the visual modality, we test a model pretrained with text inputs only. Even when this pretrained model is finetuned with both modalities, the performance is significantly lower compared to a pretrained multimodal model (last row in Table~2): there is a 25\% relative drop on all 4 metrics (\eg, 1.43 vs. 2.14 in CIDEr).
When finetuned with text inputs only, the scores drop further (\eg, to 1.20 in CIDEr). These results confirm the importance of the visual inputs during pretraining.

\begin{table}[t]
    \centering
    \scalebox{0.85}{
    \begin{tabular}{@{\hskip 0.8mm}l@{\hskip 1mm}c@{\hskip 2.5mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 0.8mm}}
    \toprule
        Method & PT parts & Inputs & B-4 & C & M & R-L \\
    \midrule 
        % Bi-LSTM~\cite{zhou2018towards} & -- & V & 0.87 & -- & 8.15 & -- \\
        % EMT~\cite{zhou2018end} & -- & V & 4.38 & 0.38 & 11.55 & 27.44 \\
        VideoBERT~\cite{sun2019videobert} & E & V & 4.04 & 0.49 & 11.01 & 27.50 \\
        % CBT~\cite{sun2019learning} & E & V & 5.12 & 0.64 & 12.97 & 30.44 \\
        ActBERT~\cite{zhu2020actbert} & E & V & 5.41 & 0.65 & 13.30 & 30.56 \\
        MART~\cite{lei2020mart} & -- & V & 8.00 & 0.36 & 15.90 & --\\
        AT~\cite{hessel2019case} & -- & T & 8.55 & 1.06 & 16.93 & 35.54 \\ 
        \hdashline
        DPC~\cite{shi2019dense} & -- & V+T & 2.76 & -- & 18.08 & -- \\
        AT+Video~\cite{hessel2019case} & -- & V+T & 9.01 & 1.12 & 17.77 & 36.65 \\ 
        % \hdashline
        DECEMBERT~\cite{tang2021decembert} & E & V+T & 11.92 & 0.58 & 20.01 & 40.22 \\
        VideoAsMT~\cite{korbar2020video} & E+D & V & 5.30 & -- & 13.40 & --\\
        M-MASS~\cite{huang2020multimodal} & E+D & V+T & 12.04 & 1.23 & 18.32 & 39.03 \\
        UniVL~\cite{luo2020univl} & E+D & V+T & 17.35 & 1.81 & 22.35 & 46.52 \\ 
        \hdashline
        MV-GPT (Ours) & E+D & V & 16.71 & 1.53 & 21.43 & 41.56 \\ % 1054K
        % MV-GPT (Ours)$\dagger$ & T* & 14.26 & 1.18 & 17.44 & 34.99 \\
        MV-GPT (Ours) & E+D & T & 16.71 & 1.56 & 20.88 & 40.19 \\ 
        \bf MV-GPT (Ours) & \bf E+D & \bf V+T & \bf 21.88 & \bf2.21 & \bf 27.09 & \bf 49.38 \\
        % \midrule
        % Human~\cite{hessel2019case} & -- & V+T & 15.20 & 3.80 & 25.90 & 45.10 \\
    \bottomrule
    \end{tabular}}
    \caption{Comparison to SOTA on YouCook2 for video captioning. 
    }
    \label{tab:sota-youcook}
\end{table}


\begin{table}[t]
    \centering
    \scalebox{0.85}{
    % \resizebox{0.99\linewidth}{!}{
    \begin{tabular}{@{\hskip 0.8mm}l@{\hskip 1mm}c@{\hskip 2.5mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 0.8mm}}
        \toprule
        Method & PT parts & Inputs&  B-1 & C & M & R-L \\
        \midrule
        M-MASS~\cite{huang2020multimodal} & E+D & V+T & 22.37 & 0.82 & 11.00 & 31.40\\ 
        \bf MV-GPT (Ours) & \bf E+D & \bf V+T & \bf 37.89 & \bf 1.04 & \bf 26.75 & \bf 34.76 \\ 
        % \midrule
        % Human~\cite{huang2020multimodal} & -- & -- & 43.34 & 1.26 & 33.56 & 41.88 \\ 
        \bottomrule
    \end{tabular}}
    \caption{Comparison to SOTA on ViTT for video captioning.}
    \label{tab:sota-vitt}
\end{table}

\begin{table}[t]
    \centering
    \scalebox{0.85}{
    % \resizebox{0.99\linewidth}{!}{
    \begin{tabular}{@{\hskip 0.8mm}l@{\hskip 1mm}c@{\hskip 2.5mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 0.8mm}}
    \toprule
        Method & PT parts & Inputs & B-4 & C & M & R-L \\
        \midrule 
        % MARN~\cite{pei2019memory} & -- & V & 40.40 & 0.47 & 28.10 & 60.70 \\
        % SibNet~\cite{liu2020sibnet} & -- & V & 40.90 & 0.48 & 27.50 & 60.20 \\
        OA-BTG~\cite{zhang2019object} & -- & V & 41.40 & 0.47 & 28.20 & -- \\
        % GRU-EVE~\cite{aafaq2019spatio} & -- & V & 38.30 & 0.48 & 28.40 & 60.70 \\
        MGSA~\cite{chen2019motion} & -- & V & 42.40 & 0.48 & 27.60 &  -- \\
        POS+CG~\cite{wang2019controllable} & -- & V & 42.00 & 0.49 & 28.20 & 61.60 \\
        POS+VCT~\cite{hou2019joint} & -- & V & 42.30 & 0.49 & 29.70 & 62.80 \\
        SAM-SS~\cite{chen2020semantics} & -- & V & 43.80 & 0.51 & 28.90 & 62.40 \\
        ORG-TRL~\cite{zhang2020object} & -- & V & 43.60 & 0.51 & 28.80 & 62.80 \\
        VNS-GRU~\cite{chen2020delving} & -- & V & 45.30 & 0.53 & 29.90 & 63.40\\ \hdashline
        DECEMBERT~\cite{tang2021decembert} & E & V & 45.20 & 0.52 & 29.70 & \bf 64.70 \\ 
        VideoAsMT~\cite{korbar2020video} & E+D & V & 41.70 & -- & 28.50 & --\\
        UniVL~\cite{luo2020univl} & E+D & V+T & 41.79 & 0.50 & 28.94 & 60.78 \\
        \hdashline
        \bf MV-GPT (Ours) & \bf E+D & \bf V+T & \bf 48.92 & \bf 0.60 & \bf 38.66 & \bf64.00 \\ 
        \bottomrule
    \end{tabular}}
    \caption{Comparison to SOTA on MSR-VTT for video captioning. }
    \label{tab:sota-msr}
\end{table}

\begin{table}[t]
    \centering
    \scalebox{0.85}{
    % \resizebox{0.99\linewidth}{!}{
    \begin{tabular}{@{\hskip 0.8mm}lcccc@{\hskip 0.8mm}}
    \toprule
        Method & B-4 & M \\
        \midrule 
        DCEV~\cite{krishna2017dense} & 1.60 & 8.88 \\
        DVC~\cite{li2018jointly} & 1.71 & 9.31 \\
        Bi-SST~\cite{wang2018bidirectional}& -- & 10.89 \\
        HACA~\cite{wang2018watch} & 2.71 & 11.16 \\
        MWSDEC~\cite{rahman2019watch} & 1.46 & 7.23 \\
        MDVC~\cite{iashin2020multi} & 1.46 & 7.23 \\
        BMT~\cite{iashin2020better} & 1.99 & 10.90 \\\hdashline
        \bf MV-GPT (Ours) & \bf 6.84 & \bf 12.31 \\ 
        \bottomrule
    \end{tabular}}
    \caption{
    Comparison to SOTA on ActivityNet-Captions for video captioning with ground-truth action proposals.}
    \label{tab:sota-activitynet}
\end{table}



\begin{figure*}
    \centering
    \scalebox{0.85}{
        \begin{tabular}{@{\hskip 0mm}c@{\hskip 4mm}c@{\hskip 0.8mm}}

            % Example1: WYAFPvlDB_A-005
            \begin{tabular}{@{\hskip 0mm}p{8.5cm}@{\hskip 2mm}p{3.3cm}@{\hskip 0.8mm}}
                \centering
                \adjincludegraphics[valign=c,width=0.48\linewidth]{figures/3_1.jpeg}~
                \adjincludegraphics[valign=c,width=0.48\linewidth]{figures/3_2.jpeg}
                &\parbox[c]{1\linewidth}{\textbf{Transcript}: 
                
                This makes a really good source. So about twenty five spice you like it. That's about 4 teaspoons}
                
            \end{tabular}
            & 
            \bgroup
            
            \begin{tabular}{@{\hskip 0mm}p{8.2cm}@{\hskip 0.8mm}}
                \raggedright \textbf{Generated captions}  \tabularnewline[1.2mm]
                \raggedright ~\colorbox[RGB]{220,230,242}{GT:} pour in spicy sauce \tabularnewline[1mm]
                \raggedright ~\colorbox[RGB]{242,220,219}{No-PT:} pour some sauce over the pasta \tabularnewline[1mm]
                \raggedright ~\colorbox[RGB]{235,241,222}{MV-GPT:} add sriracha to the bowl \tabularnewline
            \end{tabular}
            \egroup \tabularnewline[1.2cm]
            
            % Example1: video7012
            \begin{tabular}{@{\hskip 0mm}p{8.5cm}@{\hskip 2mm}p{3.3cm}@{\hskip 0.8mm}}
                \centering
                \adjincludegraphics[trim={0 1.5cm 0 0},clip,valign=c,width=0.48\linewidth]{figures/msr_video7012_1.jpeg}~
                \adjincludegraphics[trim={0 1.5cm 0 0},clip,valign=c,width=0.48\linewidth]{figures/msr_video7012_2.jpeg}
                &\parbox[c]{1\linewidth}{\textbf{Transcript}: 
                
                So by considering the whole host of nature and nurture influences, we can take a broader view of mental health ...}
                
            \end{tabular}
            & 
            \bgroup
            
            \begin{tabular}{@{\hskip 0mm}p{8.2cm}@{\hskip 0.8mm}}
                \raggedright \textbf{Generated captions}  \tabularnewline[1.2mm]
                \raggedright ~\colorbox[RGB]{220,230,242}{GT:} a man in a brown blazer discussing 
                %
                %\hspace{0.95cm}
                mental health \tabularnewline[1mm]
                \raggedright ~\colorbox[RGB]{242,220,219}{No-PT:} a man in a blue shirt is talking \tabularnewline[1mm]
                \raggedright ~\colorbox[RGB]{235,241,222}{MV-GPT:} a man in a suit is talking about mental health \tabularnewline
            \end{tabular}
            \egroup  \tabularnewline[1.25cm]

            % Example1: video7174
            \begin{tabular}{@{\hskip 0mm}p{8.5cm}@{\hskip 2mm}p{3.3cm}@{\hskip 0.8mm}}
                \centering
                \adjincludegraphics[trim={0 1.5cm 0 0.5cm},clip,valign=c,width=0.48\linewidth]{figures/msr_video7174_1.jpeg}~
                \adjincludegraphics[trim={0 1.5cm 0 0.5cm},clip,valign=c,width=0.48\linewidth]{figures/msr_video7174_2.jpeg}
                &\parbox[c]{1\linewidth}{\textbf{Transcript}: 
                
                You can take one like this.} 
                
            \end{tabular}
            & 
            \bgroup
            
            \begin{tabular}{@{\hskip 0mm}p{8.2cm}@{\hskip 0.8mm}}
                \raggedright \textbf{Generated captions}  \tabularnewline[1.2mm]
                \raggedright ~\colorbox[RGB]{220,230,242}{GT:} a person is riding a ski lift and speaking to us \tabularnewline[1mm]
                \raggedright ~\colorbox[RGB]{242,220,219}{No-PT:} a man is driving a motorcycle \tabularnewline[1mm]
                % \raggedright ~\colorbox[RGB]{242,220,219}{UniVL:} add mayo to the bowl \tabularnewline[1mm]
                \raggedright ~\colorbox[RGB]{235,241,222}{MV-GPT:} a man is walking in the woods 
            \tabularnewline
            \end{tabular}
            \egroup \\ 
        \end{tabular}
    }
    \caption{Qualitative example on YouCook2 (first row) and MSR-VTT (last two rows) including a failure case (last row). \colorbox[RGB]{220,230,242}{GT:} Ground-truth caption. \colorbox[RGB]{242,220,219}{No-PT:} No multimodal pretraining.  
    % \colorbox[RGB]{242,220,219}{UniVL:} Previous pretrained SOTA model. 
    \colorbox[RGB]{235,241,222}{MV-GPT:} Our model pretrained on HowTo100M.
    }
    \label{fig:youcook_qex}
\end{figure*}

\noindent\textbf{Comparisons to the State of the Art:} 
Finally, we compare MV-GPT to existing methods on all four datasets.
Table~\ref{tab:sota-youcook} compares our method to the state of the art on YouCook2, where we outperform all prior work including works pretrained on HowTo100M. 
On ViTT (Table~\ref{tab:sota-vitt}), the gap is even larger, with our model advancing the state-of-the-art by 15\% (absolute) compared to M-MASS in B-1 and M scores. 

Despite the domain gap between instructional videos in HowTo100M and general online videos in MSR-VTT, our model outperforms all existing work as shown in Table~\ref{tab:sota-msr}.
Although UniVL also pretrains both the encoder and the decoder on HowTo100M, our method achieves relative improvements of over 31\% thanks to our end-to-end training. 
Similarly, Table~\ref{tab:sota-activitynet} shows that our pretraining method achieves state-of-the-art performance on ActivityNet-Captions despite the significant domain gap.

\noindent\textbf{Qualitative Results:} 
We show  examples from YouCook2 and MSR-VTT in Figure~\ref{fig:youcook_qex}.
The first example illustrates that our model can use the visual modality to infer the term `sauce' despite the ASR error `\textit{source}' and further recognizes its name `\textit{sriracha}'.
Similarly, the second example illustrates that our approach manages to take into account both modalities jointly. 
Finally, we show a failure case in the last row in which our model fails to capture the concept `ski lift'.
A possible explanation is that the concept of a ski lift may be rarely seen in the pretraining dataset, a problem which may be alleviated by collecting more diverse pretraining videos, or incorporating external object knowledge through the use of pre-trained object detectors. 




\subsection{Non-generative Video Understanding Tasks}
Although MV-GPT is a generative model and is particularly designed for multimodal video captioning, we also find that our pretraining technique learns a powerful multimodal video encoder that can be transferred easily to multiple video understanding tasks.
In particular, we show results on VideoQA, video retrieval and action classification.
For details on each task please refer to the appendix.


\noindent\textbf{VideoQA:} 
We use MV-GPT as an encoder (no \texttt{BOS} token is fed to the decoder so it only contextualizes the input tokens; see appendix for details) and the average pooled input embedding is fed to a two-layered MLP classifier to predict the answer.
The question is simply concatenated to the ASR inputs.
Following the standard protocols in \cite{yang2020just,seo2021look}, we measure the answer prediction accuracy on MSRVTT-QA~\cite{xu2017video} and ActivityNet-QA~\cite{yu2019activitynet}. 

Table~\ref{tab:vqa} compares the accuracy  of MV-GPT to existing methods that are pretrained on HowTo100M~\cite{miech2019howto100m}.
Even though MV-GPT is not designed for this particular task, our model slightly outperforms the previous state-of-the-art VQA-T~\cite{yang2020just} (which is specifically designed for VideoQA) on both datasets.

%
\noindent\textbf{Video Retrieval:} 
The common practice for retrieval is to train a video-text joint embedding using \textit{discriminative} losses only, typically in the form of a standard NCE loss~\cite{gutmann2010noise}, where each video clip has a single corresponding textual caption. Here we investigate whether our generative pretraining loss can provide a boost to performance.
Since each example forms two inputs-target triplets in our bidirectional framework, we apply NCE losses on both (Bi-NCE). We then add our generative pretraining loss to this framework and report results in Table~\ref{tab:retrieval_msr}. We evaluate our model with and without ASR to compare fairly to existing works.
We report recall at $k=\{1, 5, 10\}$ (R@$k$) and median rank (MdR) on MSR-VTT~\cite{xu2016msr} following the standard 9K retrieval splits~\cite{yu2018joint}.

Our first observation is that our Bi-NCE serves as a strong baseline pretraining method for retrieval. We show that adding our generative losses further improves performance by a relative 6.3\% in R@1, yielding state-of-the-art performance.
Finally, adding ASR to our multimodal encoder further improves performance by a significant margin (+ 4\%). 


\noindent\textbf{Action Classification:} 
We test the visual encoder of \model on action classification following~\cite{arnab2021vivit}.
We evaluate models using top-1 classification accuracy on Kinetics 400 and 600~\cite{kay2017kinetics}.
Note that we adopt the ViViT-Base architecture with factorized encoder following \cite{arnab2021vivit}, however we use a tubelet size of $16\times16\times4$ instead of $16\times16\times2$ to reduce complexity.
We compare our model with two different initializations for the visual encoder: random and pretrained weights on ImageNet21k.
The baseline models are finetuned on the evaluation benchmarks immediately from these initializations whereas we first post-pretrain models in our MV-GPT framework and finetune for action classification.


Table~\ref{tab:kinetics} demonstrates that MV-GPT is an effective pretraining strategy for the visual encoder.
High-capacity transformer models like ViViT are challenging to train from scratch, and overfit easily as shown in the first row.
However, ViViT initialized from an MV-GPT visual encoder trained from scratch performs substantially better, obtaining absolute improvements of 24\% on Kinetics-400 (a standard video classification benchmark).
This number is close to  the performance of ViViT initalized with ImageNet-21K pretraining, as done by the original authors~\cite{arnab2021vivit} (note that ImageNet-21K was created with high manual annotation cost, while we used no labels at all during pretraining).
Finally, initialising the MV-GPT visual encoder with these same ImageNet-21K weights, and then pretraining the MV-GPT visual encoder weights on HowTo100M achieves the best results, improving upon the initialisation of~\cite{arnab2021vivit} by 1.5\% and 1.8\% on Kinetics-400 and Kinetics-600 respectively, which is the current state of the art on this dataset with this particular architecture.






	
\begin{table}[t]
    \centering
    \scalebox{0.8}{
    \begin{tabular}{@{\hskip 0.8mm}lcc@{\hskip 0.8mm}}
    \toprule
        Method & MSRVTT-QA & ActivityNet-QA \\
    \midrule 
        % E-SA~\cite{yu2019activitynet} & -- & 29.3 & 31.8\\
        SSML~\cite{amrani2020noise} & 35.1 & --\\
        MAR-VQA~\cite{zhuang2020multichannel} & -- & 34.6\\
        % ClipBERT~\cite{lei2021less} & COCO~\cite{chen2015microsoft}+VG~\cite{krishna2017visual} & 37.4 & --\\
        DECEMBERT~\cite{tang2021decembert} & 37.4 & -- \\
        CoMVT~\cite{seo2021look} & 39.5 & 38.8\\
        VQA-T~\cite{yang2020just} & 41.5 & 38.9 \\ \hdashline
        \bf MV-GPT (Ours) & \bf 41.7 & \bf 39.1\\% 25328956-8
    \bottomrule
    \end{tabular}}
    \caption{Comparison to SOTA on MSRVTT-QA and ActivityNet-QA for video question answering. Our method is comparable to other works, even those designed specifically for the task of VideoQA. We compare models pretrained on HowTo100M.}
    \label{tab:vqa}
\end{table}
	


\begin{table}[t]
    \centering
    \scalebox{0.85}{
    \begin{tabular}{@{\hskip 0.8mm}lccccc@{\hskip 0.8mm}}
    \toprule
        Method & With ASR & R@1 & R@5 & R@10 & MdR \\
    \midrule 
        UniVL~\cite{luo2020univl} & & 21.2 & 49.6 & 63.1 & 6 \\
        MMT~\cite{gabeur2020Learning} & & 26.6 & 57.1 & 69.6 & 4\\
        AVLnet~\cite{rouditchenko2021avlnet} & & 27.1 & 55.6 & 66.6 & 4\\
        SSB~\cite{patrick2021supportset} & & 30.1 & 58.5 & 69.3 & \bf3 \\
        HiT~\cite{liu2021hit} & & 30.7 & 60.9 & 73.2 & -- \\ \hdashline
        % \bf MV-GPT (Ours) & \bf 34.3 & \bf 62.7 & \bf 74.3 \\
        No PT & & 3.5 & 8.0 & 12.1 & 114 \\
        Bi-NCE & & 31.6 & 59.0 & 70.2 & \bf3 \\
        \bf MV-GPT (Ours) &  & \bf 33.6 & \bf 61.2 & \bf 73.6 & \bf3 \\
        \hdashline
        No PT & \checkmark & 5.6 & 13.3 & 18.4 & 92 \\
        Bi-NCE & \checkmark & 33.7 & 61.6 & 73.0 & 3 \\
        \bf MV-GPT (Ours) & \checkmark & \bf 37.3 & \bf 65.5 & \bf 75.1 & \bf2\\
    \bottomrule
    \end{tabular}}
    \caption{Comparison to SOTA on MSR-VTT for video retrieval.
    We compare models pretrained on HowTo100M. \textbf{R@$\boldsymbol{k}$}: Recall at $k$. \textbf{MdR}: Median rank. 
    %\phseo{The numbers for our model should be updated.}
    }
    \label{tab:retrieval_msr}
\end{table}



\begin{table}[t]
    \centering
    \scalebox{0.85}{
    \begin{tabular}{@{\hskip 0.8mm}lcc@{\hskip 0.8mm}}
    \toprule
        ViViT initialization & Kinetics-400 & Kinetics-600 \\ % & MSVD-QA \\
    \midrule 
         Scratch & 50.14 & 55.47 \\  %(21919230, 52), (25255668, 19)
         MV-GPT$\dagger$ & 74.20 & 77.10 \\ % (25218971, 1), (25219017, 1)
         \hdashline
         ImageNet21k~\cite{arnab2021vivit} & 78.90 & 80.62 \\     % (21356628, 13), (25219017, 4)
         ImageNet21k + MV-GPT$\dagger$ & 80.40 & 82.42 \\  % (25218971, 2) (25219017, 2)
    \bottomrule
    \end{tabular}}
    \caption{Action classification results on Kinetics with different ViViT initializations. MV-GPT$\dagger$ refers to a model initalised with our MV-GPT pretraining on HowTo100M with \textit{no manually annotated} labels. We use a  factorized encoder ViViT-Base following \cite{arnab2021vivit}, but use a tubelet size of $16\times16\times4$ instead of $16\times16\times2$.}
    \label{tab:kinetics}
    \vspace{-0.3cm}
\end{table}




==> CVPR 2022 MV-GPT for final arXiv/sections/experiments_backup.tex <==
\section{Experiments}
% This section first describes all the datasets
% used in this work, and then delves into evaluation protocols and results.

We first describe the datasets (Sec.~\ref{sec:exp_datasets}), evaluation protocols (Sec.~\ref{sec:exp_protocol}) and implementation details (Sec.~\ref{sec:exp_implementation_details}) before presenting detailed results in Sec.~\ref{sec:exp_results}.

\subsection{Datasets}
\label{sec:exp_datasets}

% \anurag{Maybe nice to indicate what tasks each dataset is used for}

\noindent\textbf{HowTo100M}~\cite{miech2019howto100m} consists of 1.2M instructional videos from YouTube. Transcribed speech is obtained using the YouTube ASR API.
Following the procedure of \cite{seo2021look}, we preprocess this dataset to extract 53M triplets of frames, current utterances and future utterances for pretraining.
%\arsha{Add exact number of triplets we train on?} % and use it for pretraining our network.

\noindent\textbf{YouCook2}~\cite{zhou2018towards} contains 2,000 cooking videos for 89 different dishes with 14K video clips. 
% The overall video duration is 176 hours (5.26 minutes per video on average). 
Each video clip is annotated with a single captioning sentence.
%We evaluate both videoQA and multimodal video captioning. \\ 

\noindent\textbf{Video Timeline Tags (ViTT)}~\cite{huang2020multimodal} 
%Given the narrow domain of YouCook2 (almost uniform distribution over 89 recipes), this dataset was 
was created 
%with videos covering a broader variety of topics 
to better reflect the distribution of instructional videos in the wild. 
It consists of 8,169 videos, 
%of which 3,381 are cooking-related.
5,840 of these videos for training and the remaining videos for validation and testing. Videos are divided into 7.1 segments on average, with each segment accompanied by a short natural language description.

\noindent\textbf{MSR-VTT}~\cite{xu2016msr} is a standard benchmark with 10K open domain video clips for both video captioning and video-retrieval.
The duration of each video clip is between 10 and 30 seconds, and 20 natural language descriptions are manually annotated per clip.
We follow the standard splits \cite{xu2016msr} and \cite{yu2018joint} for captioning and retrieval, respectively.
% For captioning, we follow the standard splits in~\cite{xu2016msr} whereas we adopt the splits used in \cite{yu2018joint} for retrieval.

\noindent\textbf{ActivityNet-Captions}~\cite{krishna2017dense} is a standard dense video captioning benchmark consisting of 100K temporally localized
sentences for 20k videos. 
We follow the standard splits with 50/25/25\% examples for training, val and test sets.
% While this benchmark requires action localization, we conduct our experiments using GT proposals.
To evaluate our model's ability to predict captions, we use ground truth temporal proposals following~\cite{krishna2017dense}.
% \anurag{Can we say ``To evaluate our model's ability to predict captions, we use ground truth temporal proposals following \cite{papers}?''} 

\noindent\textbf{MSRVTT-QA}~\cite{xu2017video} is a VideoQA benchmark derived from MSR-VTT, and contains 243K QA pairs. The dataset follows the splits in MSR-VTT.

\noindent\textbf{ActivityNet-QA}~\cite{yu2019activitynet} contains 58K QA pairs for VideoQA where the train, val and test sets have 32K, 18K and 8K pairs, respectively. 

\noindent\textbf{Kinetics}~\cite{kay2017kinetics} is the largest action classification benchmark.
We evaluate on both Kinetics 400 and 600, containing approximately 267K clips from 400 classes and 446K clips from 600 classes, respectively.
% Clips are 10-seconds long.

\subsection{Evaluation Protocols}
\label{sec:exp_protocol}

We pretrain a single model for all tasks on HowTo100M. 
While our primary focus is multimodal video captioning, we also test our pretrained multimodal or visual encoder in VideoQA, video retrieval and action classification using the following evalutation protocols.
Refer to supp. file for the details on our model architecture for each task.
Unless otherwise specified, our models are finetuned end-to-end on each target dataset.
% Detailed evaluation protocols are provided below. 


\noindent\textbf{Multimodal Video Captioning} 
For captioning, we report results in the following established metrics: BLEU-4 (B-4)~\cite{papineni2002bleu}, CIDEr (C)~\cite{vedantam2015cider}, METEOR (M)~\cite{banerjee2005meteor} and ROUGE-L (R-L)~\cite{lin2004rouge}. 
For ViTT, we measure BLEU-1 (B-1) instead of BLEU-4 following the protocol in \cite{huang2020multimodal}.

\noindent\textbf{VideoQA} 
Following previous works~\cite{yang2020just,seo2021look}, we measure the answer prediction accuracy (classification over multiple choice answers). The question is simply concatenated to the ASR inputs.
% Although we do not generate sentences, we use pooled outputs of our multimodal decoder, which are then fed to a linear classifier.
% The decoder is fed only with the multimodal context features and we place a linear classifier which takes the average pooled decoder outputs.

\noindent\textbf{Video Retrieval} 
We report recall at $k=\{1, 5, 10\}$ (R@$k$) and median rank.
We evaluate our model with and without ASR to show both fair comparisons to existing works and the best performances by our full model.
% \arsha{Mention that the decoder is not used here?}
% \anurag{+1 for being clear about which parts of the model each task evalutes.}

\noindent\textbf{Action Classification} 
We evaluate models using top-1 classification accuracy. %, by simply appending a linear classifier to the outputs of our visual encoder (all other components are not utilised).
% \anurag{Can rather justify as ``To evaluate the visual encoder learned by our pretraining objective ...'' (similar thing applies to previous paragraphs)}

\subsection{Implementation Details}
\label{sec:exp_implementation_details}

For our text encoder, we adopt the BERT-Base architecture with uncased wordpiece tokenization \cite{devlin2018bert}.
Our visual encoder uses the corresponding ViViT-Base configuration with a 1-layer temporal transformer and a tubelet size of $16\times16\times4$ \cite{arnab2021vivit}.
Our multimodal encoder consists of 2 layers following \cite{seo2021look} and finally, the decoder is based on the GPT-2 (117M parameters) architecture~\cite{radford2019language} but we modify it to take both multimodal input context $C$ and the \texttt{BOS} tokens allowing conditional generation (the original GPT starts generation immediately by taking the first word as its input and only conditions on text).
We initialize the text encoder and the decoder with standard BERT and GPT-2 weights pretrained on large-scale unlabeled corpora \cite{lu2019vilbert,radford2019language}.
Similarly, we initialize our visual encoder using the pretrained weights on Kinetics 400 in \cite{arnab2021vivit} unless otherwise specified. Our model is pretrained end-to-end using the Adam optimizer~\cite{kingma2014adam} for 1.5M iterations.
For more detailed hyperparameters and training strategies for pretraining and finetuning, please refer to the supp. document.
% with an initial learning rate of $10^{-4}$ and a batch size of 2,048. 
% We warm up linearly from 0 for 500 iterations and use cosine learning rate decay. When used, we set the weight decay factor to 0.01.
%Each pretraining takes about 1.5 weeks. \anurag{Is mentioning 1.5 weeks necessary? Also it lacks context if you don't mention the hardware being used.} 

\subsection{Results} 
\label{sec:exp_results}

In this section we ablate some key design choices, in particular the backbone and objective functions used in MV-GPT, and compare our model to the state of the art on a number of video captioning benchmarks.
Finally, we also show that our pretrained model can serve as an encoder for other tasks such as VideoQA, video retrieval and action classification. % \arsha{and retrieval?}

% \begin{table}[t]
%     \centering
%     \scalebox{0.85}{
%      \begin{tabular}{@{\hskip 0.8mm}l@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 0.8mm}}
%     \toprule
%         Losses  & B-4 & C & M & R-L \\
%     \midrule 
%  No PT & 12.49 & 0.93 & 16.07 & 34.00 \\
%  DAE + MLM (encoder) & 18.97 & 1.89 & 24.19 & 45.04 \\
%  % DAE. + MLM (decoder) + WD & 18.58 & 1.80 & 23.80 & 44.46 \\ 
%  \hdashline % 608K
%  FG + MLM (encoder) & 19.33 & 1.92 & 24.21 & 44.97 \\ % 908K
%  FG + MLM (decoder) & 19.49 & 1.95 & 24.81 & 46.09 \\
%  FG + BG + MLM (encoder) & 20.28 & 2.03 & 25.51 & 46.87 \\ % 1370K
%  FG + BG + MLM (decoder) & 20.22 & 2.05 & 25.68 & 47.37 \\ 
%  \bf FG + BG + MLM (decoder) + WD & \bf20.94 & \bf2.10 & \bf26.50 & \bf48.38 \\ 
%     \bottomrule
%     \end{tabular}}
%     \caption{Ablation on YouCook2 showing the effect of different loss functions in pretraining. \textbf{No PT:} No multimodal pretraining. \textbf{DAE:} Refers to the denoising autoencoder loss used by UniVL~\cite{luo2020univl}. \textbf{MLM:} Masked Language Modelling Loss. \textbf{FG:} Forward Generation loss. \textbf{BG:} Backward Generation loss. \textbf{WD:} Weight Decay.
%   Refer to Sec.~\ref{sec:exp_protocol} for details about evaluation metrics and Sec.~\ref{sec:abl-losses} for details about each loss.
%     } 
%     \label{tab:abl-losses}
%     % \vspace{-\baselineskip}
% \end{table}


\begin{table}[t]
    \centering
    \scalebox{0.85}{
     \begin{tabular}{@{\hskip 0.8mm}l@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 0.8mm}}
    \toprule
        Losses  & PT parts & B-4 & C & M & R-L \\
    \midrule 
 No PT & -- & 12.49 & 0.93 & 16.07 & 34.00 \\
 Baseline PT & E &  \\
 CoMVT~\cite{seo2021look} & E & 13.79 & 1.16 & 17.47 & 35.35 \\
 M-MASS~\cite{huang2020multimodal} & E+D &  \\
 UniVL~\cite{luo2020univl} & E+D & 18.97 & 1.86 & 24.35 & 45 \\
 \hdashline
 MV-GPT (Ours) & E & 15.50 & 1.37 & 20.28 & 39.94 \\
 MV-GPT (Ours) & E+D & \bf20.94 & \bf2.10 & \bf26.50 & \bf48.38 \\ 
    \bottomrule
    \end{tabular}}
    \caption{
    Comparisons to existing pretraining losses on YouCook2. 
    We reimplement the loss functions of the existing methods but use our model and training strategies for fair comparisons.
    \textbf{PT parts} shows whether the encoder (E) and the decoder (D) are pretrained. \phseo{Describe Baseline PT and M-MASS (that we are pretraining the model only with the multimodal dataset for fair comparisons.)}\phseo{Complete the missing entries.}
    } 
    \label{tab:comps-loss}
    % \vspace{-\baselineskip}
\end{table}


% \begin{table}[t]
%     \centering
%     \scalebox{0.85}{
%      \begin{tabular}{@{\hskip 0.8mm}c@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 0.8mm}}
%     \toprule
%         FG & BG & MLM-D  & B-4 & C & M & R-L \\
%     \midrule 
%  & & & 12.49 & 0.93 & 16.07 & 34.00 \\
%  \checkmark & & & 19.33 & 1.92 & 24.21 & 44.97 \\ % 908K
%  \checkmark & & \checkmark & 19.49 & 1.95 & 24.81 & 46.09 \\
%  \checkmark & \checkmark & & \bf20.28 & 2.03 & 25.51 & 46.87 \\ % 1370K
%  \checkmark & \checkmark & \checkmark & 20.22 & \bf2.05 & \bf25.68 & \bf47.37 \\ 
%     \bottomrule
%     \end{tabular}}
%     \caption{Ablation on YouCook2 showing the effect of our different loss components in pretraining. \textbf{FG:} Forward Generation loss. \textbf{BG:} Backward Generation loss. \textbf{MLM-D:} Masked Language Modelling loss applied on Decoder outputs instead of encoder outputs. 
%     % Refer to Sec.~\ref{sec:abl-losses} for details about each loss.
%     % \anurag{Why doesn't the best row correspond to Table 1?}
%     } 
%     \label{tab:abl-losses}
%     % \vspace{-\baselineskip}
% \end{table}


\begin{table}[t]
    \centering
    \scalebox{0.85}{
     \begin{tabular}{@{\hskip 0.8mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 0.8mm}}
    \toprule
        FG & BG & MLM-E & MLM-D & WD & B-4 & C & M & R-L \\
    \midrule 
 & & & & & 12.49 & 0.93 & 16.07 & 34.00 \\
 \checkmark & & \checkmark & & & 19.33 & 1.92 & 24.21 & 44.97 \\ % 908K
 \checkmark & & & \checkmark & & 19.49 & 1.95 & 24.81 & 46.09 \\
 \checkmark & \checkmark & \checkmark & & & 20.28 & 2.03 & 25.51 & 46.87 \\ % 1370K
 \checkmark & \checkmark & & \checkmark & &  20.22 & 2.05 & 25.68 & 47.37 \\ 
 \checkmark & \checkmark & & \checkmark & \checkmark & \bf20.94 & \bf2.10 & \bf26.50 & \bf48.38 \\ 
    \bottomrule
    \end{tabular}}
    \caption{Ablation on YouCook2 showing the effect of our different loss components in pretraining. \textbf{FG:} Forward Generation loss. \textbf{BG:} Backward Generation loss. \textbf{MLM-E/MLM-D:} Masked Language Modelling loss applied on encoder outputs (E) or decoder outputs (D). \textbf{WD:} Weight Decay.
    % Refer to Sec.~\ref{sec:abl-losses} for details about each loss.
    % \anurag{Why doesn't the best row correspond to Table 1?}
    } 
    \label{tab:abl-losses}
    % \vspace{-\baselineskip}
\end{table}


% \begin{table}[t]
%     \centering
%     \scalebox{0.85}{
%      \begin{tabular}{@{\hskip 0.8mm}l@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 0.8mm}}
%     \toprule
%         Losses  & B-4 & C & M & R-L \\
%     \midrule 
%  No PT & 12.15 & 0.89 & 15.91 & 32.96 \\
%  DAE + MLM (encoder) & 18.35 & 1.79 & 23.23 & 43.74 \\
%  % DAE. + MLM (decoder) + WD & 18.58 & 1.80 & 23.80 & 44.46 \\ 
%  \hdashline % 608K
%  FG + MLM (encoder) & 18.56 & 1.81 & 23.54 & 44.30 \\ % 908K
%  FG + MLM (decoder) & 19.06 & 1.88 & 24.18 & 45.15 \\
%  FG + BG + MLM (encoder) & 19.57 & 1.93 & 24.94 & 46.13 \\ % 1370K
%  FG + BG + MLM (decoder) & 19.71 & 1.98 & 25.08 & 46.62 \\ 
%  \bf FG + BG + MLM (decoder) + WD & \bf20.08 & \bf2.00 & \bf25.33 & \bf47.03 \\ 
%     \bottomrule
%     \end{tabular}}
%     \caption{Ablation on YouCook2 showing the effect of different loss functions in pretraining. \textbf{No PT:} No multimodal pretraining. \textbf{DAE:} Refers to the denoising autoencoder loss used by UniVL~\cite{luo2020univl}. \textbf{MLM:} Masked Language Modelling Loss. \textbf{FG:} Forward Generation loss. \textbf{BG:} Backward Generation loss. \textbf{WD:} Weight Decay.
%   Refer to Sec.~\ref{sec:exp_protocol} for details about evaluation metrics and Sec.~\ref{sec:abl-losses} for details about each loss.
%   \phseo{Should we redo all these ablations with Full ASR?}
%     } 
%     \label{tab:abl-losses}
%     % \vspace{-\baselineskip}
% \end{table}

% \begin{table}[t]
%     \centering
%     \scalebox{0.73}{
%      \begin{tabular}{@{\hskip 0.8mm}l@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 0.8mm}}
%     \toprule
%         Losses  & B-4 & C & M & R-L \\
%     \midrule 
%  No PT & 45.41 & 0.49 & 36.13 & 61.31 \\
%  DAE. + MLM & 47.31 & 0.57 & 37.45 & 62.93 \\
%  % DAE. + MLM (decoder) + WD & 18.58 & 1.80 & 23.80 & 44.46 \\ 
%  \hdashline % 608K
%  FG + MLM & 48.01 & 0.57 & \bf38.32 & 63.59 \\ % 908K
%  FG + MLM (decoder) & \bf48.07 & 0.58 & 37.90 & 63.59 \\
%  FG + BG + MLM & 48.16 & 0.57 & 37.79 & 63.62 \\ % 1370K
%  FG + BG + MLM (decoder) & 48.04 & \bf0.60 & 37.87 & 63.86 \\ 
%  \bf FG + BG + MLM (decoder) + WD & \bf48.07 & 0.59 & 38.12 & \bf64.01 \\ 
%     \bottomrule
%     \end{tabular}}
%     \caption{Ablation on MSR-VTT showing the effect of different loss functions in pretraining. \textbf{No PT.} No multimodal pretraining. \textbf{DAE.} Refers to the denoising autoencoder loss used by UniVL~\cite{luo2020univl}. \textbf{MLM.} Masked Language Modelling Loss. \textbf{FG.} Forward Generation loss. \textbf{BG.} Backward Generation loss. \textbf{WD.} Weight Decay. } 
%     \label{tab:abl-losses}
% \end{table}

\subsubsection{Pretraining Losses} 
\label{sec:abl-losses}
Table~\ref{tab:comps-loss} compares our proposed pretraining loss function to existing losses used in UniVL~\cite{luo2020univl} and CoMVT~\cite{seo2021look}. 
% \arsha{cite} 
We implement these losses with our model architecture for a fair comparison. 
Note that UniVL pretrains both the encoder and the decoder using five different losses whereas CoMVT pretrains only the multimodal encoder.
For CoMVT, we finetune the model with a randomly initialized decoder.
As expected, we first note that all pretraining methods significantly improve captioning performance over training from scratch. We also note that using the UniVL loss and our proposed MV-GPT loss, outperforms CoMVT with large margins. 
% \arsha{We haven't clarified here how we use CoMVT for captioning. We gotta say that we just use the encoder from CoMVT. I think it would also be good to have one line refreshing the losses in UniVL}.
Similarly, if we utilize only the encoder weights of the pretrained MV-GPT, the performance drops significantly.
This indicate the importance of the joint pretraining of the encoder and the decoder.
Finally, compared to UniVL, MV-GPT achieves relative improvements ranging from 5.8\% to 9.5\% across the four evaluation metrics thanks to the use of the future utterances and its bidirectional nature.
Note that UniVL splits a single ASR into partial signals by masking 
% \arsha{you mean by masking right? Or does partial signal mean something else here?}
to use as input and output whereas MV-GPT uses the next utterance as an additional textual supervision and mitigate the temporal mismatch 
%\anurag{Maybe I am mistaken, but this invites a comparison to MIL-NCE~\cite{miech2020end}}
through its bidirectional losses.


Table~\ref{tab:abl-losses} shows the effect of each term in our loss function.
The forward generation (FG) loss already provides strong self-supervision.
When applying the masked language modeling loss on the decoder outputs (MLM-D) instead of the encoder outputs (corresponding non-checked rows), performances are slightly improved thanks to the additional input contextualization provided by the decoder.
% Performance is slightly improved by applying the masked language modeling loss on the decoder outputs (MLM-D) instead of the encoder outputs.
% \arsha{We need to explain this better in Sec. 3.1 and then here we need to provide some reason why we think it helps}.
% \anurag{+1. Also I feel like you need to show a row with MLM-E to substantiate this}
When adopting the full bidrectional loss with the backward generation (BG), the results show significant gains on all metrics.
Additionally, we observe that adding weight decay~\cite{krogh1992simple} brings additional gains and we report our scores in this full setting for the rest of the paper.
%\anurag{Weight decay seems a bit orthogonal to the contribution of this paper. Is it possible to use weight decay everywhere, and mention this as an implementation detail?}


% the following different losses on the YouCook2 dataset.
% \textbf{No PT:} No pretraining (training the model from scratch on YouCook2), \noindent\textbf{DAE:} Denoising auto-encoder. Refers to the generative loss used by UniVL~\cite{luo2020univl}. Given a masked current utterance, we generate the unmasked sentence.  
% \noindent\textbf{FG:} Forward Generation loss. 
% \noindent\textbf{BG:} Backward Generation loss.  
% \noindent\textbf{MLM:} Masked Language Modeling. We test MLM applied in two ways - first applied only on the multimodal encoder outputs (as done in UniVL) and secondly on the decoder outputs.
% \noindent\textbf{WD:} Weight Decay.

% The results show that all pretraining ablations significantly improve model performance compared to training from scratch. We also show a qualitative result in Fig. \ref{fig:youcook_ex}.
% Although DAE pretraining improves performance over training from scratch, FG alone already outperforms DAE in most metrics, confirming our intuition that generating a new unseen utterance is a stronger form of supervision than predicting masked inputs.
% % since most of the output tokens in DAE are already given as inputs providing weaker supervisory signals to the network.
% Our bidirectional generation loss further improves the scores significantly in all metrics.
% Additionally, we observe that applying MLM on the decoder outputs works better than on the multimodal encoder outputs, signalling that the decoder can be used to learn multimodal contexualization of tokens as well as sentence generation.
% % This signifies that our decoder does not only take the role of the sentence generation but also perform the multimodal contextualization within the context inputs.
% Finally, combining all proposed losses achieves the best score, with additional improvements from using weight decay.
% This configuration is used for the rest of our experiments.
% Compared to the DAE loss of~\cite{luo2020univl}, we observe relative improvements ranging from 5.8\% to 9.5\% across the four evaluation metrics. 

% \begin{table}[t]
%     \centering
%     \scalebox{0.73}{
%     \begin{tabular}{lccccc}
%     \toprule
%         Visual Encoder & E2E & B-4 & C & M & R-L \\
%     \midrule 
% S3D (kinetics) & & 17.59 & 1.65 & 22.13 & 42.11 \\% 1254K
% S3D (HowTo100M) & & 18.03 & 1.74 & 22.79 & 43.19 \\ % 1268K
% VIVIT (scratch) & \checkmark &  19.04 & 1.85 & 24.18 & 44.91 \\ % 644K
% VIVIT (kinetics) & &  \\
% VIVIT (kinetics) & \checkmark & 20.08 & 2.00 & 25.33 & 47.03 \\
%     \bottomrule
%     \end{tabular}}
%     \caption{Ablation on YouCook2 with different visual encoder configurations. \textbf{E2E.} End-to-end training in both pretraining and finetuning.}
%     \label{tab:abl-backbone}
% \end{table}


\begin{table}[t]
    \centering
    \scalebox{0.75}{
    \begin{tabular}{@{\hskip 0.8mm}c@{\hskip 1.5mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 0.8mm}}
    \toprule
        Architecture  & Weights from & Trained on & B-4 & C & M & R-L \\
    \midrule 
S3D & S3D \cite{xie2018rethinking} & Kinetics & 18.42 & 1.80 & 23.49 & 44.02 \\% 1254K
S3D & MIL-NCE \cite{miech2020end} & HowTo100M & 19.22 & 1.89 & 24.37 & 45.23 \\ % 1268K
 \hdashline
ViViT & ViViT \cite{arnab2021vivit} & Kinetics & 18.23 & 1.77 & 23.01 & 43.37 \\
ViViT & MV-GPT (Ours)$\dagger$ & HowTo100M & 20.90 & 2.12 & 26.16 & 47.87 \\
    \bottomrule
    \end{tabular}}
    \caption{Ablation on YouCook2 with different visual encoders.
    We pretrain and finetune the other components using our method with a frozen visual encoder.
    $\dagger$ The visual encoder is learned in pretraining and is frozen in finetuning.}
    \label{tab:abl-backbone}
\end{table}


\begin{table}[t]
    \centering
    \scalebox{0.85}{
    \begin{tabular}{cccccc}
    \toprule
        Frozen VE & Frozen MME & B-4 & C & M & R-L \\
    \midrule 
    \multicolumn{6}{c}{\textit{YouCook2}} \\
    \midrule
% VIVIT (Kinetics) & & \\
 &  & \bf20.94 & 2.10 & \bf26.50 & \bf48.38 \\
\checkmark &  & 20.90 & \bf2.12 & 26.16 & 47.87 \\
\checkmark & \checkmark & 18.90 & 1.89 & 23.82 & 44.73 \\
% VIVIT (Kinetics) & Scratch D & 15.50 & 1.37 & 20.28 & 39.94 \\
    \midrule 
    \multicolumn{6}{c}{\textit{MSR-VTT}} \\
    \midrule
 & & \bf48.07 & \bf0.59 & \bf38.12 & \bf64.01 \\
\checkmark &  & 47.64 & 0.56 & 37.56 & 62.85\\
\checkmark & \checkmark & 45.94 & 0.52 & 36.88 & 61.37\\
    \bottomrule
    \end{tabular}}
    \caption{Ablation on YouCook2 and MSR-VTT freezing different modules. \textbf{Frozen MME:} Frozen multimodal encoder, only the decoder is finetuned. \textbf{Frozen VE:} The visual encoder is frozen. 
    \phseo{Add ViViT(scratch) to the appendix.}
    }
    \label{tab:abl-e2e}
\end{table}


% \begin{table}[t]
%     \centering
%     \scalebox{0.7}{
%     \begin{tabular}{lcccccc}
%     \toprule
%         Visual Encoder & E2E PT & E2E FT & B-4 & C & M & R-L \\
%     \midrule 
%     \multicolumn{7}{c}{\textit{YouCook2}} \\
%     \midrule
% S3D (Kinetics) & Frozen VE & Frozen VE & 18.42 & 1.80 & 23.49 & 44.02 \\% 1254K
% S3D (HowTo100M) & Frozen VE & Frozen VE & 19.22 & 1.89 & 24.37 & 45.23 \\ % 1268K
% VIVIT (Scratch) & \checkmark & \checkmark & 19.95 & 2.00 & 25.26 & 46.59 \\ % 644K
% % VIVIT (Kinetics) & & \\
% VIVIT (Kinetics) & \checkmark & Frozen MME & 18.90 & 1.89 & 23.82 & 44.73 \\
% VIVIT (Kinetics) & Frozen VE & Frozen VE & 18.23 & 1.77 & 23.01 & 43.37 \\
% VIVIT (Kinetics) & \checkmark & Frozen VE & 20.90 & 2.12 & 26.16 & 47.87 \\
% \color{red} VIVIT (Kinetics) & \checkmark & Scratch D & 15.50 & 1.37 & 20.28 & 39.94 \\
% VIVIT (Kinetics) & \checkmark & \checkmark & 20.94 & 2.10 & 26.50 & 48.38 \\
%     \midrule 
%     \multicolumn{7}{c}{\textit{MSR-VTT}} \\
%     \midrule
% VIVIT (Kinetics) & \checkmark & Frozen VE & 47.64 & 0.56 & 37.56 & 62.85\\
% VIVIT (Kinetics) & \checkmark & \checkmark & 48.07 & 0.59 & 38.12 & 64.01 \\
%     \bottomrule
%     \end{tabular}}
%     \caption{Ablation on YouCook2 and MSR-VTT with different visual encoders. \textbf{E2E PT:} End-to-end pretraining. \textbf{E2E FT:} End-to-end finetuning. \textbf{Frozen MME:} Frozen multimodal encoder, only the decoder is finetuned. \textbf{Frozen VE:} Only the visual encoder is frozen. A \checkmark indicates all weights are updated during training.}
%     \label{tab:abl-backbone}
% \end{table}



% \begin{table}[t]
%     \centering
%     \scalebox{0.7}{
%     \begin{tabular}{lcccccc}
%     \toprule
%         Visual Encoder & E2E PT & E2E FT & B-4 & C & M & R-L \\
%     \midrule 
%     \multicolumn{7}{c}{\textit{YouCook2}} \\
%     \midrule
% S3D (Kinetics) & Frozen VE & Frozen VE & 17.59 & 1.65 & 22.13 & 42.11 \\% 1254K
% S3D (HowTo100M) & Frozen VE & Frozen VE & 18.03 & 1.74 & 22.79 & 43.19 \\ % 1268K
% VIVIT (Scratch) & \checkmark & \checkmark & 19.04 & 1.85 & 24.18 & 44.91 \\ % 644K
% % VIVIT (Kinetics) & & \\
% VIVIT (Kinetics) & \checkmark & Frozen MME & 18.37 & 1.81 & 23.36 & 44.07 \\
% VIVIT (Kinetics) & Frozen VE & Frozen VE & 17.59 & 1.68 & 21.94 & 41.81 \\
% VIVIT (Kinetics) & \checkmark & Frozen VE & 20.32 & 2.02 & 25.32 & 46.73 \\
% \color{red} VIVIT (Kinetics) & \checkmark & Scratch D & 15.50 & 1.37 & 20.28 & 39.94 \\
% VIVIT (Kinetics) & \checkmark & \checkmark & 20.94 & 2.10 & 26.50 & 48.38 \\
%     \midrule 
%     \multicolumn{7}{c}{\textit{MSR-VTT}} \\
%     \midrule
% VIVIT (Kinetics) & \checkmark & Frozen VE & 48.19 & 0.55 & 37.41 & 62.73\\
% VIVIT (Kinetics) & \checkmark & \checkmark & 48.07 & 0.59 & 38.12 & 64.01 \\
%     \bottomrule
%     \end{tabular}}
%     \caption{Ablation on YouCook2 and MSR-VTT with different visual encoders. \textbf{E2E PT:} End-to-end pretraining. \textbf{E2E FT:} End-to-end finetuning. \textbf{Frozen MME:} Frozen multimodal encoder, only the decoder is finetuned. \textbf{Frozen VE:} Only the visual encoder is frozen. A \checkmark indicates all weights are updated during training.}
%     \label{tab:abl-backbone}
% \end{table}

% \begin{table}[t]
%     \centering
%     \scalebox{0.63}{
%     \begin{tabular}{lcccccc}
%     \toprule
%         Visual Encoder & E2E PT & E2E FT & B-4 & C & M & R-L \\
%     \midrule 
% VIVIT (kinetics) & \checkmark & No vis enc & 48.19 & 0.55 & 37.41 & 62.73\\
% VIVIT (kinetics) & \checkmark & \checkmark & 48.07 & 0.59 & 38.12 & 64.01 \\
%     \bottomrule
%     \end{tabular}}
%     \caption{Ablation on MSR-VTT with different visual encoder configurations.}
%     \label{tab:abl-backbone-msrvtt}
% \end{table}

% \begin{table}[t]
%     \centering
%     \scalebox{0.63}{
%     \begin{tabular}{lcccccc}
%     \toprule
%         Visual Encoder & E2E PT & E2E FT & B-4 & C & M & R-L \\
%     \midrule 
% S3D (kinetics) & & & 46.56 & 0.54 & 36.87 & 62.56 \\
% S3D (HowTo100M) & & & 44.45 & 48.12 & 35.66 & 60.75 \\ % 1268K
% VIVIT (scratch) & \checkmark & \checkmark & 45.99 & 0.54 & 36.47 & 62.44 \\ % 644K
% VIVIT (kinetics) & & \\
% VIVIT (kinetics) & \checkmark & Dec only & 45.94 & 0.52 & 36.88 & 61.37 \\
% VIVIT (kinetics) & \checkmark & No vis enc & 48.19 & 0.55 & 37.41 & 62.73\\
% VIVIT (kinetics) & \checkmark & \checkmark & 48.07 & 0.59 & 38.12 & 64.01 \\
%     \bottomrule
%     \end{tabular}}
%     \caption{Ablation on MSR-VTT with different visual encoder configurations.}
%     \label{tab:abl-backbone-msrvtt}
% \end{table}

\subsubsection{Visual Encoder and End-to-end Training} 
In Table~\ref{tab:abl-backbone}, we first compare the ViViT~\cite{arnab2021vivit} encoder to commonly used S3D features~\cite{xie2018rethinking}.
When both encoders are trained on Kinetics and fixed for multimodal pretraining and finetuning, they show comparable scores despite the large complexity of S3D due to the high frame rate required (30 fps vs. 1 fps for ViViT).
Using HowTo100M to train a visual encoder, we observe large gains with both architectures as expected given the similarity in domains -- HowTo100M and YouCook2 are both instructional video datasets.
However, we observe larger gains with ViViT when the visual encoder is optimized for  generative losses within our framework and jointly trained with the other components thanks to its low complexity.
These results show the benefits of end-to-end pretraining.

% In Table~\ref{tab:abl-backbone}, we compare the ViViT~\cite{arnab2021vivit} encoder to commonly used S3D features~\cite{xie2018rethinking}.
% S3D features trained on HowTo100M as in \cite{miech2020end} outperform those trained on Kinetics (as expected given the similarity in domain - HowTo100M and YouCook2 are both instructional video datasets). In both cases the S3D features are frozen, because end-to-end training with S3D features is computationally infeasible on long videos given the high frame rate of consecutive frames required (30 fps). Using a ViViT encoder trained from scratch leads to improved results, despite the coarse frame sampling and the fact that there is no initialisation \eg\ from Kinetics. This is further improved by initialising the visual encoder with weights from a Kinetics-400 trained model.

We further investigate the importance of end-to-end training in Table~\ref{tab:abl-e2e}.
We freeze some components such as the visual encoder while finetuning the other components, which is the setting commonly adopted in all previous approaches for multimodal video pretraining~\cite{luo2020univl,li2020hero, tang2021decembert,huang2020multimodal}.
When we freeze the visual encoder, we get similar performance on YouCook2, but the performance drop on MSR-VTT -- this is because end-to-end training allows our model to better adapt to the target domain (which is different for MSR-VTT as it does not consist of instructional videos).
If we freeze the entire multimodal encoder and finetune the decoder only, the performance drops further on both datasets.
% \anurag{We never say ``performances''}


% If we freeze only the visual encoder, we get similar performance on YouCook2, but performance drops on MSR-VTT -- this is because end-to-end training allows our model to better adapt to the target domain (which is different for MSR-VTT as it does not consist of instructional videos). 
% We also note that finetuning the decoder only gives worse performance than finetuning the entire model.
% \red{
% Finally, if we use the pretrained weights to initialize only the multimodal encoder and train the decoder from scratch during the finetuning\footnote{We still initialize the decoder using pretrained GPT-2 weights on the text dataset.}, the performance drops significantly. This indicates the importance of the joint pretraining of both encoder and decoder for captioning, and shows the limitation of the encoder-only pretraining techniques.
% }


\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/scale_eval.png}
    \caption{Performance changes in four captioning metrics with varying pretraining dataset sizes on YouCook2 for video captioning. }
    \label{fig:scale}
\end{figure}

\subsubsection{Dataset Sizes and Multimodality}
Figure~\ref{fig:scale} reports performance against dataset size. 
All four metrics show improvement (almost linear) when the dataset size is doubled. 
This signifies the potential gains from collecting more unlabeled videos for pretraining. 
% \arsha{We need something to say here. Hence we would expect further performance gains with more data? Performance is not yet saturated?}
% \anurag{Yes, but this could also suggest that you need a lot more data to get a small improvement. So don't know if its worth mentioning}
% \phseo{Should we move this to the supplementary?}


\begin{table}[t]
    \centering
    \scalebox{0.85}{
    \begin{tabular}{@{\hskip 0.8mm}l@{\hskip 1mm}c@{\hskip 2.5mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 0.8mm}}
    \toprule
        Method & PT parts & Inputs & B-4 & C & M & R-L \\
    \midrule 
        Bi-LSTM~\cite{zhou2018towards} & -- & V & 0.87 & -- & 8.15 & -- \\
        EMT~\cite{zhou2018end} & -- & V & 4.38 & 0.38 & 11.55 & 27.44 \\
        VideoBERT~\cite{sun2019videobert} & E & V & 4.04 & 0.49 & 11.01 & 27.50 \\
        CBT~\cite{sun2019learning} & E & V & 5.12 & 0.64 & 12.97 & 30.44 \\
        ActBERT~\cite{zhu2020actbert} & E & V & 5.41 & 0.65 & 13.30 & 30.56 \\
        VideoAsMT~\cite{korbar2020video} & E & V & 5.30 & -- & 13.40 & --\\
        MART~\cite{lei2020mart} & -- & V & 8.00 & 0.36 & 15.90 & --\\
        AT~\cite{hessel2019case} & -- & T & 8.55 & 1.06 & 16.93 & 35.54 \\ 
        \hdashline
        DPC~\cite{shi2019dense} & -- & V+T & 2.76 & -- & 18.08 & -- \\
        AT+Video~\cite{hessel2019case} & -- & V+T & 9.01 & 1.12 & 17.77 & 36.65 \\ 
        % \hdashline
        DECEMBERT~\cite{tang2021decembert} & E & V+T & 11.92 & 0.58 & 20.01 & 40.22 \\
        M-MASS~\cite{huang2020multimodal} & E+D & V+T & 12.04 & 1.23 & 18.32 & 39.03 \\
        UniVL~\cite{luo2020univl} & E+D & V+T & 17.35 & 1.81 & 22.35 & 46.52 \\ 
        \hdashline
        MV-GPT (Ours) & E+D & V & 16.71 & 1.53 & 21.43 & 41.56 \\ % 1054K
        % MV-GPT (Ours)$\dagger$ & T* & 14.26 & 1.18 & 17.44 & 34.99 \\
        MV-GPT (Ours) & E+D & T & 15.49 & 1.40 & 19.71 &     37.82 \\ 
        \bf MV-GPT (Ours) & \bf E+D & \bf V+T & \bf 20.94 & \bf2.10 & \bf 26.50 & \bf 48.38 \\ \midrule
        Human~\cite{hessel2019case} & -- & V+T & 15.20 & 3.80 & 25.90 & 45.10 \\
    \bottomrule
    \end{tabular}}
    \caption{Comparison to SOTA on YouCook2 for video captioning. 
    }
    \label{tab:sota-youcook}
\end{table}

% \subsubsection{Multimodal vs Single Modality}
In Table~\ref{tab:sota-youcook}, we show results with text only and visual only inputs (we just feed the \texttt{CLS} token for the omitted modality). It is clear that both modalities are complementary and performance is best when combining both.
% We note that our vision-only model performs better than the text-only model -- however this is because we were unable to obtain ASR transcripts for all the videos in the YouCook2 validation set. We conjecture that all our results could be further improved if we had access to the ASR for all videos, as used in other works.
% We conjecture that our visual encoder is tuned end-to-end and the model relies more on the visual inputs.

\begin{table}[t]
    \centering
    \scalebox{0.85}{
    % \resizebox{0.99\linewidth}{!}{
    \begin{tabular}{@{\hskip 0.8mm}l@{\hskip 1mm}c@{\hskip 2.5mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 0.8mm}}
        \toprule
        Method & PT parts & Inputs&  B-1 & C & M & R-L \\
        \midrule
        M-MASS~\cite{huang2020multimodal} & E+D & V+T & 22.37 & 0.82 & 11.00 & 31.40\\ 
        \bf MV-GPT (Ours) &E+D & V+T & \bf 37.89 & \bf 1.04 & \bf 26.75 & \bf 34.76 \\ 
        \midrule
        Human~\cite{huang2020multimodal} & 43.34 & 1.26 & 33.56 & 41.88 \\ 
        \bottomrule
    \end{tabular}}
    \caption{Comparison to SOTA on ViTT for video captioning.}
    \label{tab:sota-vitt}
\end{table}

\begin{table}[t]
    \centering
    \scalebox{0.85}{
    % \resizebox{0.99\linewidth}{!}{
    \begin{tabular}{@{\hskip 0.8mm}l@{\hskip 1mm}c@{\hskip 2.5mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 0.8mm}}
    \toprule
        Method & PT parts & Inputs & B-4 & C & M & R-L \\
        \midrule 
        MARN~\cite{pei2019memory} & -- & V & 40.40 & 0.47 & 28.10 & 60.70 \\
        SibNet~\cite{liu2020sibnet} & -- & V & 40.90 & 0.48 & 27.50 & 60.20 \\
        OA-BTG~\cite{zhang2019object} & -- & V & 41.40 & 0.47 & 28.20 & -- \\
        GRU-EVE~\cite{aafaq2019spatio} & -- & V & 38.30 & 0.48 & 28.40 & 60.70 \\
        MGSA~\cite{chen2019motion} & -- & V & 42.40 & 0.48 & 27.60 &  -- \\
        POS+CG~\cite{wang2019controllable} & -- & V & 42.00 & 0.49 & 28.20 & 61.60 \\
        POS+VCT~\cite{hou2019joint} & -- & V & 42.30 & 0.49 & 29.70 & 62.80 \\
        SAM-SS~\cite{chen2020semantics} & -- & V & 43.80 & 0.51 & 28.90 & 62.40 \\
        ORG-TRL~\cite{zhang2020object} & -- & V & 43.60 & 0.51 & 28.80 & 62.80 \\
        VNS-GRU~\cite{chen2020delving} & -- & V & 45.30 & 0.53 & 29.90 & 63.40\\ \hdashline
        DECEMBERT~\cite{tang2021decembert} & E & V & 45.20 & 0.52 & 29.70 & \bf 64.70 \\ 
        UniVL~\cite{luo2020univl} & E+D & V+T & 41.79 & 0.50 & 28.94 & 60.78 \\
        \hdashline
        \bf MV-GPT (Ours) & E+D & V+T & \bf 48.07 & \bf 0.59 & \bf 38.12 & 64.01 \\ 
        \bottomrule
    \end{tabular}}
    \caption{Comparison to SOTA on MSR-VTT for video captioning. $\dagger$ Models pretrained on HowTo100M.}
    \label{tab:sota-msr}
\end{table}

\begin{table}[t]
    \centering
    \scalebox{0.85}{
    % \resizebox{0.99\linewidth}{!}{
    \begin{tabular}{@{\hskip 0.8mm}lcccc@{\hskip 0.8mm}}
    \toprule
        Method & B-4 & M \\
        \midrule 
        DCEV~\cite{krishna2017dense} & 1.60 & 8.88 \\
        DVC~\cite{li2018jointly} & 1.71 & 9.31 \\
        Bi-SST~\cite{wang2018bidirectional}& -- & 10.89 \\
        HACA~\cite{wang2018watch} & 2.71 & 11.16 \\
        MWSDEC~\cite{rahman2019watch} & 1.46 & 7.23 \\
        MDVC~\cite{iashin2020multi} & 1.46 & 7.23 \\
        BMT~\cite{iashin2020better} & 1.99 & 10.90 \\\hdashline
        \bf MV-GPT (Ours) & \bf 6.84 & \bf 12.31 \\ 
        \bottomrule
    \end{tabular}}
    \caption{
    Comparison to SOTA on ActivityNet-Captions for video captioning with ground-truth action proposals.}
    \label{tab:sota-activitynet}
\end{table}



\begin{figure*}
    \centering
    \scalebox{0.85}{
        \begin{tabular}{@{\hskip 0.8mm}c@{\hskip 7mm}c@{\hskip 0.8mm}}

            % Example1: WYAFPvlDB_A-005
            \begin{tabular}{@{\hskip 0.8mm}p{9cm}@{\hskip 2mm}p{4.3cm}@{\hskip 0.8mm}}
                \centering
                \adjincludegraphics[valign=c,width=0.48\linewidth]{figures/3_1.jpeg}~
                \adjincludegraphics[valign=c,width=0.48\linewidth]{figures/3_2.jpeg}
                &\parbox[c]{1\linewidth}{\textbf{Transcript}: This makes a really good source. So about twenty five spice you like it. That's about 4 teaspoons where take your tuna.}
                
            \end{tabular}
            & 
            \bgroup
            
            \begin{tabular}{@{\hskip 0mm}l@{\hskip 0.8mm}}
                \raggedright \textbf{Generated captions}  \tabularnewline[1.2mm]
                \raggedright ~\colorbox[RGB]{220,230,242}{GT:} pour in spicy sauce \tabularnewline[1mm]
                \raggedright ~\colorbox[RGB]{242,220,219}{No-PT:} pour some sauce over the pasta \tabularnewline[1mm]
                \raggedright ~\colorbox[RGB]{242,220,219}{UniVL:} add mayo to the bowl \tabularnewline[1mm]
                \raggedright ~\colorbox[RGB]{235,241,222}{MV-GPT:} add sriracha to the bowl \tabularnewline
            \end{tabular}
            \egroup \\ 
    
        \end{tabular}
    }
    \caption{Qualitative example on YouCook2. \colorbox[RGB]{220,230,242}{GT:} Ground-truth caption. \colorbox[RGB]{242,220,219}{No-PT:} No multimodal pretraining on HowTo100M. \colorbox[RGB]{242,220,219}{UniVL:} Previous pretrained SOTA model. \colorbox[RGB]{235,241,222}{MV-GPT:} Our pretrained model. Despite the ASR error \textit{sauce}$\rightarrow$\textit{source}, our model is able to generate the precise name of the sauce from the input frames.
    In contrast, UniVL misrecognizes the sauce as 'mayo' and No-PT erroneously generates the word 'pasta'.
    %, unlike the model without pretraining which erroneously generates the word `pasta'.
    }
    \label{fig:youcook_ex}
\end{figure*}

\subsubsection{Comparisons to the State of the Art} 
%\noindent\textbf{Video Captioning:} 
Table~\ref{tab:sota-youcook} compares our method to state of the art works on YouCook2. 
Our method outperforms all prior work, including M-MASS and UniVL which also both pretrain on HowTo100M. % \anurag{This makes it sound like M-MASS and UniVL are the only comparable works in the table}. 
On ViTT (Table~\ref{tab:sota-vitt}), the gaps are even larger, with our model advancing the state-of-the-art by 15\% (absolute) compared to M-MASS in the BLEU-1 and Meteor scores. %\anurag{Why is the gap so much larger on this dataset? Because of the end-to-end training of the visual encoder?}
%achieveing the state of the art results by ~15\% absolute improvement over M-MASS in the BLEU-1 and Meteor scores.

Despite the domain gap between instructional videos in the pretraining dataset and general online videos in MSR-VTT, our model outperforms all existing work in most of the metrics as shown in Table~\ref{tab:sota-msr}.
% For a fair comparison, we obtain the scores of UniVL on MSR-VTT using the author's code\footnote{\url{https://github.com/microsoft/UniVL}}. 
Although they also use HowTo100M for pretraining, our method achieves relative improvements of over 31\% thanks to our end-to-end training. %\anurag{of the visual encoder?}.
Similarly, Table~\ref{tab:sota-activitynet} shows that our pretraining method achieves the state-of-the-art performances on ActivityNet-Captions despite the significant domain gap.
We show qualitative results in Figure~\ref{fig:youcook_ex}.

% {
% \color{red}
% \subsubsection{Efficient Transfer to Captioning}
% \phseo{Test the captioning performances with zero-shot / few-shot settings.
% Add the results to Table 3 and 5.
% If the results present good performances, it can be because the model already produces content-related captions but their styles are different (pragmatic vs. narrative). }
% }

	
\begin{table}[t]
    \centering
    \scalebox{0.8}{
    \begin{tabular}{@{\hskip 0.8mm}l@{\hskip 1mm}c@{\hskip 0mm}c@{\hskip 2mm}c@{\hskip 0.8mm}}
    \toprule
        Method & Pretrained on & MSRVTT-QA & ActivityNet-QA \\
    \midrule 
        E-SA~\cite{yu2019activitynet} & -- & 29.3 & 31.8\\
        SSML~\cite{amrani2020noise} & HowTo100M~\cite{miech2019howto100m} & 35.1 & --\\
        MAR-VQA~\cite{zhuang2020multichannel} & -- & -- & 34.6\\
        ClipBERT~\cite{lei2021less} & COCO~\cite{chen2015microsoft}+VG~\cite{krishna2017visual} & 37.4 & --\\
        DECEMBERT~\cite{tang2021decembert} & HowTo100M~\cite{miech2019howto100m} & 37.4 & -- \\
        CoMVT~\cite{seo2021look} & HowTo100M~\cite{miech2019howto100m} & 39.5 & 38.8\\
        VQA-T~\cite{yang2020just} &  HowToVQA~\cite{yang2020just} & 41.5 & 38.9 \\ \hdashline
        \bf MV-GPT (Ours) & \textbf{HowTo100M}~\cite{miech2019howto100m} & \bf 41.7 & \bf 39.1\\% 25328956-8
    \bottomrule
    \end{tabular}}
    \caption{Comparison to SOTA on MSRVTT-QA and ActivityNet-QA for video question answering. Our method is comparable to other works, even those designed specifically for the task of VideoQA.}
    \label{tab:vqa}
\end{table}
\subsubsection{MV-GPT as a Multimodal Encoder}
Although MV-GPT is a generative model, we also test it as a multimodal video encoder, specifically for the task of video question answering (VideoQA) on MSRVTT-QA and ActivityNet-QA (Table~\ref{tab:vqa}). 
% \arsha{It's not clear exactly how this is trained, we don't have the decoder at all here right? Or do we train with the generative losses as well for retrieval?}
% We test our model for VideoQA on MSRVTT-QA and ActivityNet-QA and Table~\ref{tab:vqa} compares our model to the previous state of the art methods.
Even though MV-GPT is not designed for this particular task, our model slightly outperforms the previous state-of-the-art VQA-T~\cite{yang2020just} (which is specifically designed for VideoQA) on both datasets.
% Although MV-GPT is not designed for this particular task, our model slightly outperforms on both benchmarks the best existing model VQA-T, which pretrains specifically targeting VideoQA only.
% \phseo{add details to the supplementary}


\begin{table}[t]
    \centering
    \scalebox{0.85}{
    \begin{tabular}{@{\hskip 0.8mm}lcccc@{\hskip 0.8mm}}
    \toprule
        Method & R@1 & R@5 & R@10 & MdR \\
    \midrule 
        UniVL~\cite{luo2020univl} & 21.2 & 49.6 & 63.1 & 6 \\
        MMT~\cite{gabeur2020Learning} & 26.6 & 57.1 & 69.6 & 4\\
        AVLnet~\cite{rouditchenko2021avlnet} & 27.1 & 55.6 & 66.6 & 4\\
        SSB~\cite{patrick2021supportset} & 30.1 & 58.5 & 69.3 & \bf3 \\
        HiT~\cite{liu2021hit} & 30.7 & 60.9 & 73.2 & -- \\ \hdashline
        % \bf MV-GPT (Ours) & \bf 34.3 & \bf 62.7 & \bf 74.3 \\
        \bf MV-GPT w/o ASR (Ours) & \bf 33.6 & \bf 61.2 & \bf 73.6 & \bf3 \\
        \bf MV-GPT w/ ASR (Ours) & \bf 37.3 & \bf 65.5 & \bf 75.1 & \bf2\\
    \bottomrule
    \end{tabular}}
    \caption{Comparison to SOTA on MSR-VTT for video retrieval.
    We compare models pretrained on HowTo100M. \textbf{R@$\boldsymbol{k}$}: Recall at $k$. \textbf{MdR}: Median rank. 
    %\phseo{The numbers for our model should be updated.}
    }
    \label{tab:retrieval_msr}
\end{table}

Similarly, we also evaluate our multimodal encoder for the video retrieval task on MSR-VTT. 
We pretrain our model with an additional NCE loss and a textual encoder to enforce a joint embedding space between multimodal videos and text queries. 
For detailed settings, refer to the supplementary.
Table~\ref{tab:retrieval_msr} clearly shows that MV-GPT outperforms the existing models in the fair configuration.
Moreover, feeding ASR to our multimodal encoder further improves the performance.

% \arsha{I think potentially reviewers might ask for performance without HowTo100M pretraining, to see how much gain comes from pretraining and how much from our model architecture}.


\subsubsection{MV-GPT as Cross-modal Pretraining}
Finally, Table~\ref{tab:kinetics} demonstrates that MV-GPT is an effective pretraining strategy for the visual encoder.
High-capacity transformer models like ViViT are challenging to train from scratch, and overfit easily as shown in the first row.
However, ViVIT initialised from an MV-GPT visual encoder trained from scratch performs substantially better, obtaining absolute improvements of 24\% on Kinetics-400 (a standard video classification benchmark).
This figure approaches the performance of ViViT initalized with ImageNet-21K pretraining, as done by the original authors~\cite{arnab2021vivit} (note that ImageNet-21K was created with high manual annotation cost, while we used no labels at all during pretraining).
Finally, initialising the MV-GPT visual encoder with these same ImageNet-21K weights, and then pretraining the MV-GPT visual encoder weights on HowTo100M achieves the best results, improving upon the initialisation of~\cite{arnab2021vivit} by 1.5\% and 1.8\% on Kinetics-400 and Kinetics-600 respectively, which is the current state of the art on this dataset with this model.
% Table~\ref{tab:kinetics} therefore demonstrates that our pretraining process learns strong visual representations from unlabelled videos.

\iffalse
    Finally, Table~\ref{tab:kinetics} presents the of the same ViViT architecture on Kinetics~\cite{kay2017kinetics}, \anurag{the largest dataset for action classification}, with different initializations.
    When ViViT is initialized the visual encoder weights of \model pretrained from scratch (ViViT+MV-GPT), this already gives more than 20\% absolute improvements in both Kinetics 400 and 600 compared to ViViT-scratch, which is trained from scratch.
    Note that ViViT+MV-GPT does not use any labeled datasets.
    Even when we use an additional labeled dataset, \cs{check refernce} ImageNet21k~\cite{deng2009imagenet}, to initialize ViViT as in \cite{arnab2021vivit}, we find that our pretraining still improves the quality of the visual representation by more than 1\% of accuracy.
    These results clearly indicate that our pretraining process learns strong visual representations from unlabeled videos.
    \anurag{Maybe emphasise that - 
    	High capacity models like ViViT overfit easily, so very challenging to train from scratch.
    	MV-GPT pre-training allows one to train ViViT from scratch, and finetune on Kinetics.
    	The result of this approaches ViViT initialised from an ImageNet-21K pretrained model as used by~\cite{arnab2021vivit}.
    	Best results are obtained if the ViViT part of MV-GPT is initialised from an ImageNet-21K model, trained in a self-supervised fashion, and then finetuned on Kinetics.
    }
    \todo{distinguish between name of model, and name of pretraining strategy}

\begin{table}[t]
    \centering
    \scalebox{0.73}{
    \begin{tabular}{@{\hskip 0.8mm}lcc@{\hskip 0.8mm}}
    \toprule
        ViViT initialization & Kinetics-400 & Kinetics-600 \\ % & MSVD-QA \\
    \midrule 
         ViViT-scratch & 47.46 & ~55.xx \\  %(21919230, 52), (25255668, 19)
         ViViT+MV-GPT$\dagger$ & 71.88 & 75.69 \\ % (25218971, 1), (25219017, 1)
         ViViT+ImageNet21k & 76.93 & 79.74 \\     % (21356628, 13), (25219017, 4)
         ViViT+ImageNet21k+MV-GPT$\dagger$ & 78.73 & 81.10 \\  % (25218971, 2) (25219017, 2)
        % None & & 41.5 \\ % & 46.3 \\
        % Ours \\
    \bottomrule
    \end{tabular}}
    \caption{Action classification results on Kinetics with different ViViT initialization. $\dagger$\model refers to initialization from our visual encoder weights in \model pretrained on HowTo100M with \textit{no action classification} labels.}
    \label{tab:kinetics}
\end{table}
\fi

\begin{table}[t]
    \centering
    \scalebox{0.85}{
    \begin{tabular}{@{\hskip 0.8mm}lcc@{\hskip 0.8mm}}
    \toprule
        ViViT initialization & Kinetics-400 & Kinetics-600 \\ % & MSVD-QA \\
    \midrule 
         Scratch & 50.14 & 55.47 \\  %(21919230, 52), (25255668, 19)
         MV-GPT$\dagger$ & 74.20 & 77.10 \\ % (25218971, 1), (25219017, 1)
         \hdashline
         ImageNet21k~\cite{arnab2021vivit} & 78.90 & 80.62 \\     % (21356628, 13), (25219017, 4)
         ImageNet21k + MV-GPT$\dagger$ & 80.40 & 82.42 \\  % (25218971, 2) (25219017, 2)
        % None & & 41.5 \\ % & 46.3 \\
        % Ours \\
    \bottomrule
    \end{tabular}}
    \caption{Action classification results on Kinetics with different ViViT initializations. MV-GPT$\dagger$ refers to a model initalised with our MV-GPT pretraining on HowTo100M with \textit{no manually annotated} labels.}
    \label{tab:kinetics}
\end{table}


==> CVPR 2022 MV-GPT for final arXiv/sections/intro.tex <==
\section{Introduction}

A long-standing goal of the AI community is the development of conversational multimodal systems that can both reliably perceive the world and effortlessly communicate with humans. 
An emerging benchmark of progress in this field is the task of multimodal video captioning~\cite{huang2020multimodal,luo2020univl} - which tests both abilities; a successful model must not only accurately understand \textit{`multimodal'} streams of input video (including the speech and the video frames), but also generate coherent natural language descriptions of the content.



Unsurprisingly, a major challenge in the field of vision and language learning is the lack of large-scale, manually annotated data. Annotating captions for videos is time intensive, expensive and subjective (with low inter-annotator agreement~\cite{huang2020multimodal}) -- this is in contrast to fields such as image classification where fully annotated datasets are orders of magnitude larger~\cite{ILSVRC15,hinton2015distilling,yalniz2019billion}. 
To overcome this limitation, there has been a flurry of recent works that pretrain their video-language models on instructional videos~\cite{sun2019videobert,sun2019learning,miech2020end,luo2020univl,seo2021look}, a domain where the speech is particularly well aligned to visual content.
Recently introduced datasets such as Cooking312K~\cite{sun2019videobert} and HowTo100M~\cite{miech2019howto100m} leverage such instructional videos with associated captions from ASR (automatic speech recognition) to learn joint video-and-text embeddings~\cite{sun2019learning,miech2020end} or to train multimodal video encoders~\cite{li2020hero,seo2021look}.
However, the models in these works often do not contain a decoder, lacking the ability to generate sentences, and thus only the video encoder is transferred to the downstream tasks -- indeed for the case of video captioning, the decoder is often learned from scratch~\cite{tang2021decembert,sun2019videobert,zhu2020actbert}.
While one can still initialize the decoder using independently pretrained weights such as those from a GPT-2~\cite{radford2019language} model, we observe that this strategy is suboptimal and performance is significantly improved by optimizing the encoder and the decoder jointly.


\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figures/pretraining.png}
    \caption{\textbf{Multimodal Video Generative Pretraining (MV-GPT) framework.}
    During pretraining, our network (which consists of 
    modality specific encoders, a multimodal encoder and a sentence decoder)
    is trained with a new bi-directional objective.
    1) Forward generation ({\bf FG}, \colorbox[RGB]{220,230,242}{blue}): Given input frames and present utterances from a video clip, we predict a future utterance and 2) Backward generation ({\bf BG}, \colorbox[RGB]{242,220,219}{red}): Given input frames and a future utterance, predict the current utterances. Both losses are applied to a triplet consisting of video frames, present utterances and a future utterance. 
    To allow our model to recognise the different configurations, we attach distinct special classification tokens \texttt{CLS1} and \texttt{CLS2} to the input text for FG and BG respectively, as well as distinct \texttt{BOS1} and \texttt{BOS2} (beginning of sentence) tokens to the decoder for sentence generation.
	}
    \label{fig:framework}
    \vspace{-0.1cm}
\end{figure*}
For the task of multimodal video captioning, we require a model that can both encode multimodal videos (\ie frames and textual inputs) \textit{and} generate captions. Using multimodal information as input can greatly improve the quality of the generated captions (as illustrated in Figure~\ref{fig:teaser1}). 
However, learning such 
an encoder-decoder model jointly
from unlabelled data is particularly challenging, as it requires two streams of textual data -- naturally occurring transcribed speech accompanying the video for the encoder, and target sentences for the decoder -- whereas unlabelled videos only come with a single stream of speech (Figure~\ref{fig:teaser2}).
%
Recent works~\cite{korbar2020video,luo2020univl, huang2020multimodal} have attempted to solve this problem 
with a denoising autoencoder - wherein the input speech to the model is artificially \textit{`noised'}, \ie random words are masked out~\cite{korbar2020video,luo2020univl, huang2020multimodal}. The decoder is then tasked with simply reconstructing either the masked phrases or the original unmasked text, where the supervisory signals are provided only from the masked words.
In these frameworks, additional losses are often required to strengthen the pretraining supervision, such as multimodal input alignment~\cite{luo2020univl} and segment ordering~\cite{huang2020multimodal}. 

In our framework, we introduce a novel stronger loss. We leverage future utterances as another source of textual data and train a model to generate these entirely unseen sentences as depicted in Figure~\ref{fig:teaser2}.
To alleviate the problem that future utterances are not temporally aligned,
we propose a
backward generation objective where present aligned utterances are generated given future utterances.
Experimental results show that a model pretrained with this bidirectional generation objective effectively transfers to  multimodal video captioning and outperforms the state of the art by a margin. 



We make the following contributions: 
(i) We propose a novel pretraining objective for multimodal video captioning that requires no manually annotated captions, and instead uses utterances sampled at different times in the same video. Our objective is bidirectional in time -- \ie we not only generate future utterances but also the present ones from the future;
(ii) By using two sources of textual data, we are able to jointly train the entire encoder-decoder model. This is unlike previous works which pretrain only the (multimodal) encoder, thereby lacking the ability to generate captions~\cite{seo2021look,sun2019videobert,li2020hero};
(iii) Our encoder is trained from raw pixels and words directly, in contrast with existing methods that rely on pre-extracted visual features limiting transfer to new domains~\cite{luo2020univl,korbar2020video,huang2020multimodal};
(iv) We achieve state-of-the-art results on four video captioning benchmarks -- YouCook2, ViTT, MSR-VTT and ActivityNet-Captions -- 
consistently outperforming existing methods by significant margins; and finally
(v) Our pretraining objective yields strong multimodal video representations, which achieve state-of-the-art performance on other video understanding tasks such as VideoQA, video retrieval and action classification.


==> CVPR 2022 MV-GPT for final arXiv/sections/method.tex <==
\section{Method}
Our objective is to pretrain a model that can effectively encode multimodal videos (visual frames and transcribed speech) as well as decode natural language sentences. This will allow us to use the model for multimodal captioning.
In this section, we first describe the pretraining losses used to train the encoder and decoder jointly from unlabelled videos.
We then describe our model, which consists of modality specific encoders, a multimodal encoder and a text decoder (Figure~\ref{fig:framework}).

 
\subsection{Pretraining Objectives and Losses} 
Our framework is designed to take advantage of unlabelled instructional video data, which consists of video frames and utterances often linked to the visual content~\cite{miech2019howto100m}.
As mentioned earlier, our framework requires two textual streams -- an input to the encoder and a captioning target for the decoder. Because unlabelled videos do not have captioning targets, 
we instead propose a simple objective -- our model is trained to generate a \textit{future} utterance in the video given the current video context and current utterances (forward generation). This gives us two sources of textual supervision, the current utterance allows us to learn how to optimally fuse modalities in the video encoder, while the decoder is tasked with predicting a new utterance it has never seen before. However, our goal is video captioning, and not `predicting the future'. 
To enable our model to generate text corresponding to the present video context, we also add in an additional backward generation loss -- where the model must generate the current utterance given the current video frames and a future utterance (backward generation). This encourages generated sentences to be temporally aligned (and hence more tightly coupled) with the visual inputs.



\subsubsection{Bi-directional Utterance Generation} 
Given a large set of unlabelled videos, we extract short clips consisting of visual frames $F=\{f_1,\dots,f_{N_f}\}$ and transcribed speech utterances $U=\{u_1,\dots,u_{N_u}\}$ aligned with $F$. For each clip, we also consider the immediate future utterance $W=\{w_1,\dots,w_{N_w}\}$ where $u_i$ and $w_j$ are tokenized words in the transcribed utterances. 
Note that we use the term `utterance' to refer to a single sentence of transcribed speech. 
	
\noindent\textbf{Forward Generation:}
Our model is trained to generate a future utterance $W$ given clip frames $F$ and present utterances $U$.
Formally speaking, we formulate our forward generation objective to minimize the negative log-likelihood of the true future utterance $W$, where the loss function given by the chain rule is $\mathcal{L}_\mathrm{FG}=-\sum_{i=1}^{N_w}{\log P(w_i|w_1,\dots,w_{i-1}, F, U)}$.
This loss encourages the pretrained model to effectively encode temporally aligned multimodal inputs to predict the future utterance.

\noindent\textbf{Backward Generation:}
We now apply the same loss as above, albeit in the backward direction. 
Namely, the model is tasked with generating present utterances $U$ aligned with video frames $F$, conditioned on future utterances $W$ and $F$.
As in the forward generation, we also minimize the negative log-likelihood of the true present utterance $\mathcal{L}_\mathrm{BG}=-\sum_{i=1}^{N_u}\log P(u_i|u_1,\dots,u_{i-1}, F, W)$.
Note that the visual input $F$ is temporally aligned with the decoder output $U$.
This loss function encourages the network to generate a caption related to the visual contents.

\subsubsection{Masked Language Modeling}
\label{sec:mlm}
As an additional supplementary loss, we also train with a masked language modeling (MLM) loss~\cite{devlin2018bert}
$\mathcal{L}_\mathrm{MLM}(X)$ where $X$ is the input utterance on which the masking is applied.
We apply this loss on both the forward and backward input utterances, \ie\ as $\mathcal{L}_\mathrm{MLM}(U)$ and $\mathcal{L}_\mathrm{MLM}(W)$.
Note that these losses are computed independently from the above bidirectional generation losses.

Unlike UniVL~\cite{luo2020univl} where the MLM loss is applied to the outputs of the encoder, we apply it to the outputs of the decoder. This encourages the self attention layers in the decoder to focus on further multimodal contextualization of the textual tokens (since each masked token prediction requires knowledge of neighbouring context). As we show in the experiments, this leads to performance gains.






\subsection{Model} \label{sec:architecture}
Our model consists entirely of transformer blocks, and is trained end-to-end directly from pixels and word tokens. 

\subsubsection{Modality Specific Encoders}
Given a multimodal video input consisting of the visual frames $F=\{f_1,\dots,f_{N_f}\}$ and text inputs $X=\{x_1,\dots,x_{N_x}\}$, we first extract features from the individual modalities independently. 
Note here that the textual input $X$ is the aligned utterance $U$ in general (for computing the forward generation loss and for downstream captioning tasks) but is set to $W$ when computing the backward generation loss.

\noindent\textbf{Textual Encoder:} 
We extract $N_x$ contextualized textual embeddings $E=\{e_i\}$ from the input text using a BERT~\cite{devlin2018bert} encoder.

\noindent\textbf{Visual Encoder:} 
Unlike previous approaches~\cite{sun2019videobert, luo2020univl, huang2020multimodal, seo2021look} where visual features are pre-extracted by models pretrained on different datasets, we extract the visual features directly from pixels.
We use the recent transformer-based video encoder ViViT~\cite{arnab2021vivit}, in particular, the tubelet embedding scheme and the factorized encoder architecture. 
For the tubelet embedding scheme we first extract spatio-temporal 3D tubes from the visual input volume resulting in $S\times T$ token embeddings where $S$ and $T$ correspond to the numbers of tokens in the spatial and temporal dimensions, respectively.
Then, the spatial transformer first takes each group of $S$ embeddings from the same temporal index with a special \texttt{CLS} token embedding, and the temporal transformer models interactions between the output \texttt{CLS} embeddings of the individual spatial groups with another \texttt{CLS} embedding resulting in $T+1$ visual features $V=\{v_j\}$ -- see \cite{arnab2021vivit} for further details. 

Unlike 3D CNN visual encoders which operate on consecutive frames extracted at high frame rates (30 fps), our visual encoder can operate on coarsely sampled frames (1 fps), thus significantly reducing compute. This allows us to train the visual encoder end-to-end, and helps adapt our features across the domain gaps between pretraining and downstream datasets. It also allows the easy adoption of off-the-shelf video augmentation directly to RGB frames, which is useful for small-scale downstream benchmarks.

\subsubsection{Multimodal Encoder}
Once the two sets of textual features $E$ and visual features $V$ are extracted, our multimodal encoder fuses multimodal information using the co-attentional transformer used in \cite{lu2019vilbert,seo2021look}.
Each layer consists of two streams where each stream is a stack of two transformer blocks.
In the textual stream, we first contextualize the features $E$ using a cross-attention transformer block attending to the visual features $V$.
Then, the output features are further contextualized by another transformer block with self-attention.
The first transformer block performs inter-modality contextualization through a cross-attention process whereas the second transformer block carries out intra-modality contextualization through a self-attention process.
In the same way, the visual stream $V$ attends to the textual stream. 
Our multimodal encoder repeats this process $R$ times resulting in the output multimodal features $\hat{E}$ and $\hat{V}$.



\subsubsection{Sentence Decoder}
As shown in Figure~\ref{fig:framework}, given multimodal video features $C=\hat{E}\cup \hat{V}$ as context, we autoregressively generate the output sentence $Y$ conditioned on this context using a transformer decoder.
To generate token $y_i$, we first encode the previous generated tokens $Y_i=\{y_{0}, \dots, y_{i-1}\}$ with a look-up table and a positional embedding to produce $H_i=\{h_{0}, \dots, h_{i-1}\}$.
We then encode the context $C$ and the previous embedded tokens $H_i$ using a single transformer. The outputs of this transformer are $\Tilde{C} \cup \Tilde{H}_i$, where $\Tilde{H}_i=\{\Tilde{h}_0,\dots,\Tilde{h}_{i-1}\}$.
Note that $\Tilde{C}$ refers to the multimodal input embeddings obtained from the decoder and is used for computing the MLM loss as discussed in Section~\ref{sec:mlm}.
%
We then predict the next token $y_i$ from $\Tilde{h}_{i-1}$ by a linear projection with a softmax: $y_i = \mathrm{argmax}(\mathrm{softmax}(\Phi \Tilde{h}_{i-1}))$, where $\Phi \in \mathbb{R}^{\nu\times d}$ is the linear projection matrix and $\nu$ is the vocabulary size.
The first word $h_0$ is set using the special \texttt{BOS} (beginning of sentence) token, and tokens are generated until a special \texttt{EOS} (end of sentence) token is generated.
In practice, each iteration requires only a single forward pass on the decoder transformer with the aid of causal masking introduced in~\cite{vaswani2017attention}. 

\subsubsection{Input and Output Configurations}
\noindent\textbf{Pretraining:} 
Since our pretraining objective is bidirectional, each triplet $(F, U, W)$ consisting of the visual frames $F$, the present utterances $U$ and the future utterance $W$ is processed by the network twice.
For forward generation, the model takes $F$ and $U$ as inputs and generates $W$, and it generates $U$ given $F$ and $W$, in backward generation.
To enable the model to recognize the different configurations, we attach distinct, special tokens \texttt{CLS1} and \texttt{CLS2} to the input text for the forward and backward generation losses respectively as illustrated in Figure~\ref{fig:framework}.
Similarly, we feed distinct \texttt{BOS1} and \texttt{BOS2} tokens to the decoder to initiate sentence generation.

\noindent\textbf{Finetuning for captioning:}
In downstream video captioning datasets, video clips (consisting of frames $F$ and aligned utterances $U$) are manually annotated with a natural language caption.
During finetuning, we attach the \texttt{CLS1} token to $U$ (as is done in forward generation), since $U$ is an aligned utterance, but for generation we feed in the \texttt{BOS2} token (as is done in backward generation to predict the present utterance), so that we also generate a temporally aligned caption.
\vspace{-0.05\baselineskip}  



\subsubsection{Implementation Details}

For our text encoder, we adopt the BERT-Base architecture with uncased wordpiece tokenization \cite{devlin2018bert}.
Our visual encoder uses the corresponding ViViT-Base configuration with a 1-layer temporal transformer and a tubelet size of $16\times16\times4$ \cite{arnab2021vivit}.
Our multimodal encoder consists of 2 layers following \cite{seo2021look} and finally, the decoder is based on the GPT-2 (117M parameters) architecture~\cite{radford2019language} but we modify it to take both multimodal input context $C$ and a \texttt{BOS} token allowing conditional generation (the original GPT starts generation immediately by taking the first word as its input and only conditions on text).
We initialize the text encoder and the decoder with the standard BERT and GPT-2 weights respectively pretrained on large-scale unlabelled corpora \cite{devlin2018bert,radford2019language}.
Similarly, we initialize our visual encoder using the pretrained weights on Kinetics 400 in \cite{arnab2021vivit} unless otherwise specified. Our model is pretrained end-to-end using the Adam optimizer~\cite{kingma2014adam} for 1.5M iterations with the batch size of 2048.
For more detailed hyperparameters and training strategies for pretraining and finetuning, please refer to the appendix.


==> CVPR 2022 MV-GPT for final arXiv/sections/related.tex <==
\section{Related Work}

\noindent {\bf Video captioning.} Early works in video captioning consisted of rule-based methods~\cite{kojima2002natural,das2013thousand}, where subjects, verbs and objects (SVO-triplets) detected from the video were combined into sentence templates. Later work moved away from rule-based methods by framing captioning as a machine translation task~\cite{rohrbach2013translating,sutskever2014sequence,bahdanau2015neural}, which developed the common encoder-decoder paradigm of today for the task -- the encoder processes a set of video features and accumulates its hidden state, which is then passed to a decoder for
producing a caption.
% https://arxiv.org/pdf/2101.05806.pdf 
Early works implemented the visual encoder as a 2D CNN (either frozen or finetuned) applied to video frames, which was then naturally extended to 3D CNNs~\cite{carreira2017quo,xie2018rethinking}, to better capture motion dynamics, with temporal aggregation over the entire video typically performed using attention strategies~\cite{chen2019motion}. Given the computational challenge of using expensive 3D CNNs applied to dense frame inputs (typically 30 fps), most of these works operated on pre-extracted features, only learning the fusion of features in the encoder. Unlike such works, we address this problem using a transformer-based encoder applied to raw pixels~\cite{arnab2021vivit}, sampled at a coarse rate to better capture long range context. 

\noindent {\bf Pretraining with weakly paired data.} 
Existing video captioning datasets~\cite{xu2016msr,zhou2018towards,huang2020multimodal} are orders of magnitude smaller than video classification datasets~\cite{kay2017kinetics}. As a source of weakly paired video and language data, a number of works have used the visual frames and the Automatic Speed Recognition (ASR) transcripts of unlabelled videos to pretrain video representations~\cite{sun2019videobert,sun2019learning,miech2020end,zhu2020actbert,li2020hero,seo2021look}.
These approaches learn multimodal representations by formulating proxy tasks such as masked language/frame modeling~\cite{sun2019videobert,seo2021look}, video-text matching~\cite{miech2020end,li2020hero} or segment ordering~\cite{li2020hero}.
While these studies show improvements on visual representation~\cite{sun2019videobert,sun2019learning,miech2020end,tang2021decembert} or multimodal video representation~\cite{li2020hero,zhu2020actbert,seo2021look} learning, they are designed for discriminative tasks only, and lack the generation capability. 
Pretraining techniques for generative tasks such as ours, are fewer. While \cite{korbar2020video} use multimodal translation as a generative objective, their encoder is limited to accept visual inputs only.
Works that use multimodal inputs to the encoder, train with masking losses -- wherein words or phrases are masked and the objective is to reconstruct the original sentences~\cite{korbar2020video,luo2020univl} or the masked targets~\cite{huang2020multimodal} using an autoregressive generator.
In contrast, we make use of utterances outside of the clip boundary, which are simply ignored in previous works.
We leverage 
future utterances as a second source 
of textual data, and propose a bi-directional generation objective where the model generates the future utterance given the current utterance and vice versa. While we also use a masked language modelling loss, this is simply in addition to our primary generative bidirectional loss.







==> sections/experiments_backup.tex <==
\section{Experiments}
% This section first describes all the datasets
% used in this work, and then delves into evaluation protocols and results.

We first describe the datasets (Sec.~\ref{sec:exp_datasets}), evaluation protocols (Sec.~\ref{sec:exp_protocol}) and implementation details (Sec.~\ref{sec:exp_implementation_details}) before presenting detailed results in Sec.~\ref{sec:exp_results}.

\subsection{Datasets}
\label{sec:exp_datasets}

% \anurag{Maybe nice to indicate what tasks each dataset is used for}

\noindent\textbf{HowTo100M}~\cite{miech2019howto100m} consists of 1.2M instructional videos from YouTube. Transcribed speech is obtained using the YouTube ASR API.
Following the procedure of \cite{seo2021look}, we preprocess this dataset to extract 53M triplets of frames, current utterances and future utterances for pretraining.
%\arsha{Add exact number of triplets we train on?} % and use it for pretraining our network.

\noindent\textbf{YouCook2}~\cite{zhou2018towards} contains 2,000 cooking videos for 89 different dishes with 14K video clips. 
% The overall video duration is 176 hours (5.26 minutes per video on average). 
Each video clip is annotated with a single captioning sentence.
%We evaluate both videoQA and multimodal video captioning. \\ 

\noindent\textbf{Video Timeline Tags (ViTT)}~\cite{huang2020multimodal} 
%Given the narrow domain of YouCook2 (almost uniform distribution over 89 recipes), this dataset was 
was created 
%with videos covering a broader variety of topics 
to better reflect the distribution of instructional videos in the wild. 
It consists of 8,169 videos, 
%of which 3,381 are cooking-related.
5,840 of these videos for training and the remaining videos for validation and testing. Videos are divided into 7.1 segments on average, with each segment accompanied by a short natural language description.

\noindent\textbf{MSR-VTT}~\cite{xu2016msr} is a standard benchmark with 10K open domain video clips for both video captioning and video-retrieval.
The duration of each video clip is between 10 and 30 seconds, and 20 natural language descriptions are manually annotated per clip.
We follow the standard splits \cite{xu2016msr} and \cite{yu2018joint} for captioning and retrieval, respectively.
% For captioning, we follow the standard splits in~\cite{xu2016msr} whereas we adopt the splits used in \cite{yu2018joint} for retrieval.

\noindent\textbf{ActivityNet-Captions}~\cite{krishna2017dense} is a standard dense video captioning benchmark consisting of 100K temporally localized
sentences for 20k videos. 
We follow the standard splits with 50/25/25\% examples for training, val and test sets.
% While this benchmark requires action localization, we conduct our experiments using GT proposals.
To evaluate our model's ability to predict captions, we use ground truth temporal proposals following~\cite{krishna2017dense}.
% \anurag{Can we say ``To evaluate our model's ability to predict captions, we use ground truth temporal proposals following \cite{papers}?''} 

\noindent\textbf{MSRVTT-QA}~\cite{xu2017video} is a VideoQA benchmark derived from MSR-VTT, and contains 243K QA pairs. The dataset follows the splits in MSR-VTT.

\noindent\textbf{ActivityNet-QA}~\cite{yu2019activitynet} contains 58K QA pairs for VideoQA where the train, val and test sets have 32K, 18K and 8K pairs, respectively. 

\noindent\textbf{Kinetics}~\cite{kay2017kinetics} is the largest action classification benchmark.
We evaluate on both Kinetics 400 and 600, containing approximately 267K clips from 400 classes and 446K clips from 600 classes, respectively.
% Clips are 10-seconds long.

\subsection{Evaluation Protocols}
\label{sec:exp_protocol}

We pretrain a single model for all tasks on HowTo100M. 
While our primary focus is multimodal video captioning, we also test our pretrained multimodal or visual encoder in VideoQA, video retrieval and action classification using the following evalutation protocols.
Refer to supp. file for the details on our model architecture for each task.
Unless otherwise specified, our models are finetuned end-to-end on each target dataset.
% Detailed evaluation protocols are provided below. 


\noindent\textbf{Multimodal Video Captioning} 
For captioning, we report results in the following established metrics: BLEU-4 (B-4)~\cite{papineni2002bleu}, CIDEr (C)~\cite{vedantam2015cider}, METEOR (M)~\cite{banerjee2005meteor} and ROUGE-L (R-L)~\cite{lin2004rouge}. 
For ViTT, we measure BLEU-1 (B-1) instead of BLEU-4 following the protocol in \cite{huang2020multimodal}.

\noindent\textbf{VideoQA} 
Following previous works~\cite{yang2020just,seo2021look}, we measure the answer prediction accuracy (classification over multiple choice answers). The question is simply concatenated to the ASR inputs.
% Although we do not generate sentences, we use pooled outputs of our multimodal decoder, which are then fed to a linear classifier.
% The decoder is fed only with the multimodal context features and we place a linear classifier which takes the average pooled decoder outputs.

\noindent\textbf{Video Retrieval} 
We report recall at $k=\{1, 5, 10\}$ (R@$k$) and median rank.
We evaluate our model with and without ASR to show both fair comparisons to existing works and the best performances by our full model.
% \arsha{Mention that the decoder is not used here?}
% \anurag{+1 for being clear about which parts of the model each task evalutes.}

\noindent\textbf{Action Classification} 
We evaluate models using top-1 classification accuracy. %, by simply appending a linear classifier to the outputs of our visual encoder (all other components are not utilised).
% \anurag{Can rather justify as ``To evaluate the visual encoder learned by our pretraining objective ...'' (similar thing applies to previous paragraphs)}

\subsection{Implementation Details}
\label{sec:exp_implementation_details}

For our text encoder, we adopt the BERT-Base architecture with uncased wordpiece tokenization \cite{devlin2018bert}.
Our visual encoder uses the corresponding ViViT-Base configuration with a 1-layer temporal transformer and a tubelet size of $16\times16\times4$ \cite{arnab2021vivit}.
Our multimodal encoder consists of 2 layers following \cite{seo2021look} and finally, the decoder is based on the GPT-2 (117M parameters) architecture~\cite{radford2019language} but we modify it to take both multimodal input context $C$ and the \texttt{BOS} tokens allowing conditional generation (the original GPT starts generation immediately by taking the first word as its input and only conditions on text).
We initialize the text encoder and the decoder with standard BERT and GPT-2 weights pretrained on large-scale unlabeled corpora \cite{lu2019vilbert,radford2019language}.
Similarly, we initialize our visual encoder using the pretrained weights on Kinetics 400 in \cite{arnab2021vivit} unless otherwise specified. Our model is pretrained end-to-end using the Adam optimizer~\cite{kingma2014adam} for 1.5M iterations.
For more detailed hyperparameters and training strategies for pretraining and finetuning, please refer to the supp. document.
% with an initial learning rate of $10^{-4}$ and a batch size of 2,048. 
% We warm up linearly from 0 for 500 iterations and use cosine learning rate decay. When used, we set the weight decay factor to 0.01.
%Each pretraining takes about 1.5 weeks. \anurag{Is mentioning 1.5 weeks necessary? Also it lacks context if you don't mention the hardware being used.} 

\subsection{Results} 
\label{sec:exp_results}

In this section we ablate some key design choices, in particular the backbone and objective functions used in MV-GPT, and compare our model to the state of the art on a number of video captioning benchmarks.
Finally, we also show that our pretrained model can serve as an encoder for other tasks such as VideoQA, video retrieval and action classification. % \arsha{and retrieval?}

% \begin{table}[t]
%     \centering
%     \scalebox{0.85}{
%      \begin{tabular}{@{\hskip 0.8mm}l@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 0.8mm}}
%     \toprule
%         Losses  & B-4 & C & M & R-L \\
%     \midrule 
%  No PT & 12.49 & 0.93 & 16.07 & 34.00 \\
%  DAE + MLM (encoder) & 18.97 & 1.89 & 24.19 & 45.04 \\
%  % DAE. + MLM (decoder) + WD & 18.58 & 1.80 & 23.80 & 44.46 \\ 
%  \hdashline % 608K
%  FG + MLM (encoder) & 19.33 & 1.92 & 24.21 & 44.97 \\ % 908K
%  FG + MLM (decoder) & 19.49 & 1.95 & 24.81 & 46.09 \\
%  FG + BG + MLM (encoder) & 20.28 & 2.03 & 25.51 & 46.87 \\ % 1370K
%  FG + BG + MLM (decoder) & 20.22 & 2.05 & 25.68 & 47.37 \\ 
%  \bf FG + BG + MLM (decoder) + WD & \bf20.94 & \bf2.10 & \bf26.50 & \bf48.38 \\ 
%     \bottomrule
%     \end{tabular}}
%     \caption{Ablation on YouCook2 showing the effect of different loss functions in pretraining. \textbf{No PT:} No multimodal pretraining. \textbf{DAE:} Refers to the denoising autoencoder loss used by UniVL~\cite{luo2020univl}. \textbf{MLM:} Masked Language Modelling Loss. \textbf{FG:} Forward Generation loss. \textbf{BG:} Backward Generation loss. \textbf{WD:} Weight Decay.
%   Refer to Sec.~\ref{sec:exp_protocol} for details about evaluation metrics and Sec.~\ref{sec:abl-losses} for details about each loss.
%     } 
%     \label{tab:abl-losses}
%     % \vspace{-\baselineskip}
% \end{table}


\begin{table}[t]
    \centering
    \scalebox{0.85}{
     \begin{tabular}{@{\hskip 0.8mm}l@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 0.8mm}}
    \toprule
        Losses  & PT parts & B-4 & C & M & R-L \\
    \midrule 
 No PT & -- & 12.49 & 0.93 & 16.07 & 34.00 \\
 Baseline PT & E &  \\
 CoMVT~\cite{seo2021look} & E & 13.79 & 1.16 & 17.47 & 35.35 \\
 M-MASS~\cite{huang2020multimodal} & E+D &  \\
 UniVL~\cite{luo2020univl} & E+D & 18.97 & 1.86 & 24.35 & 45 \\
 \hdashline
 MV-GPT (Ours) & E & 15.50 & 1.37 & 20.28 & 39.94 \\
 MV-GPT (Ours) & E+D & \bf20.94 & \bf2.10 & \bf26.50 & \bf48.38 \\ 
    \bottomrule
    \end{tabular}}
    \caption{
    Comparisons to existing pretraining losses on YouCook2. 
    We reimplement the loss functions of the existing methods but use our model and training strategies for fair comparisons.
    \textbf{PT parts} shows whether the encoder (E) and the decoder (D) are pretrained. \phseo{Describe Baseline PT and M-MASS (that we are pretraining the model only with the multimodal dataset for fair comparisons.)}\phseo{Complete the missing entries.}
    } 
    \label{tab:comps-loss}
    % \vspace{-\baselineskip}
\end{table}


% \begin{table}[t]
%     \centering
%     \scalebox{0.85}{
%      \begin{tabular}{@{\hskip 0.8mm}c@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 0.8mm}}
%     \toprule
%         FG & BG & MLM-D  & B-4 & C & M & R-L \\
%     \midrule 
%  & & & 12.49 & 0.93 & 16.07 & 34.00 \\
%  \checkmark & & & 19.33 & 1.92 & 24.21 & 44.97 \\ % 908K
%  \checkmark & & \checkmark & 19.49 & 1.95 & 24.81 & 46.09 \\
%  \checkmark & \checkmark & & \bf20.28 & 2.03 & 25.51 & 46.87 \\ % 1370K
%  \checkmark & \checkmark & \checkmark & 20.22 & \bf2.05 & \bf25.68 & \bf47.37 \\ 
%     \bottomrule
%     \end{tabular}}
%     \caption{Ablation on YouCook2 showing the effect of our different loss components in pretraining. \textbf{FG:} Forward Generation loss. \textbf{BG:} Backward Generation loss. \textbf{MLM-D:} Masked Language Modelling loss applied on Decoder outputs instead of encoder outputs. 
%     % Refer to Sec.~\ref{sec:abl-losses} for details about each loss.
%     % \anurag{Why doesn't the best row correspond to Table 1?}
%     } 
%     \label{tab:abl-losses}
%     % \vspace{-\baselineskip}
% \end{table}


\begin{table}[t]
    \centering
    \scalebox{0.85}{
     \begin{tabular}{@{\hskip 0.8mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 0.8mm}}
    \toprule
        FG & BG & MLM-E & MLM-D & WD & B-4 & C & M & R-L \\
    \midrule 
 & & & & & 12.49 & 0.93 & 16.07 & 34.00 \\
 \checkmark & & \checkmark & & & 19.33 & 1.92 & 24.21 & 44.97 \\ % 908K
 \checkmark & & & \checkmark & & 19.49 & 1.95 & 24.81 & 46.09 \\
 \checkmark & \checkmark & \checkmark & & & 20.28 & 2.03 & 25.51 & 46.87 \\ % 1370K
 \checkmark & \checkmark & & \checkmark & &  20.22 & 2.05 & 25.68 & 47.37 \\ 
 \checkmark & \checkmark & & \checkmark & \checkmark & \bf20.94 & \bf2.10 & \bf26.50 & \bf48.38 \\ 
    \bottomrule
    \end{tabular}}
    \caption{Ablation on YouCook2 showing the effect of our different loss components in pretraining. \textbf{FG:} Forward Generation loss. \textbf{BG:} Backward Generation loss. \textbf{MLM-E/MLM-D:} Masked Language Modelling loss applied on encoder outputs (E) or decoder outputs (D). \textbf{WD:} Weight Decay.
    % Refer to Sec.~\ref{sec:abl-losses} for details about each loss.
    % \anurag{Why doesn't the best row correspond to Table 1?}
    } 
    \label{tab:abl-losses}
    % \vspace{-\baselineskip}
\end{table}


% \begin{table}[t]
%     \centering
%     \scalebox{0.85}{
%      \begin{tabular}{@{\hskip 0.8mm}l@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 0.8mm}}
%     \toprule
%         Losses  & B-4 & C & M & R-L \\
%     \midrule 
%  No PT & 12.15 & 0.89 & 15.91 & 32.96 \\
%  DAE + MLM (encoder) & 18.35 & 1.79 & 23.23 & 43.74 \\
%  % DAE. + MLM (decoder) + WD & 18.58 & 1.80 & 23.80 & 44.46 \\ 
%  \hdashline % 608K
%  FG + MLM (encoder) & 18.56 & 1.81 & 23.54 & 44.30 \\ % 908K
%  FG + MLM (decoder) & 19.06 & 1.88 & 24.18 & 45.15 \\
%  FG + BG + MLM (encoder) & 19.57 & 1.93 & 24.94 & 46.13 \\ % 1370K
%  FG + BG + MLM (decoder) & 19.71 & 1.98 & 25.08 & 46.62 \\ 
%  \bf FG + BG + MLM (decoder) + WD & \bf20.08 & \bf2.00 & \bf25.33 & \bf47.03 \\ 
%     \bottomrule
%     \end{tabular}}
%     \caption{Ablation on YouCook2 showing the effect of different loss functions in pretraining. \textbf{No PT:} No multimodal pretraining. \textbf{DAE:} Refers to the denoising autoencoder loss used by UniVL~\cite{luo2020univl}. \textbf{MLM:} Masked Language Modelling Loss. \textbf{FG:} Forward Generation loss. \textbf{BG:} Backward Generation loss. \textbf{WD:} Weight Decay.
%   Refer to Sec.~\ref{sec:exp_protocol} for details about evaluation metrics and Sec.~\ref{sec:abl-losses} for details about each loss.
%   \phseo{Should we redo all these ablations with Full ASR?}
%     } 
%     \label{tab:abl-losses}
%     % \vspace{-\baselineskip}
% \end{table}

% \begin{table}[t]
%     \centering
%     \scalebox{0.73}{
%      \begin{tabular}{@{\hskip 0.8mm}l@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 3.5mm}c@{\hskip 0.8mm}}
%     \toprule
%         Losses  & B-4 & C & M & R-L \\
%     \midrule 
%  No PT & 45.41 & 0.49 & 36.13 & 61.31 \\
%  DAE. + MLM & 47.31 & 0.57 & 37.45 & 62.93 \\
%  % DAE. + MLM (decoder) + WD & 18.58 & 1.80 & 23.80 & 44.46 \\ 
%  \hdashline % 608K
%  FG + MLM & 48.01 & 0.57 & \bf38.32 & 63.59 \\ % 908K
%  FG + MLM (decoder) & \bf48.07 & 0.58 & 37.90 & 63.59 \\
%  FG + BG + MLM & 48.16 & 0.57 & 37.79 & 63.62 \\ % 1370K
%  FG + BG + MLM (decoder) & 48.04 & \bf0.60 & 37.87 & 63.86 \\ 
%  \bf FG + BG + MLM (decoder) + WD & \bf48.07 & 0.59 & 38.12 & \bf64.01 \\ 
%     \bottomrule
%     \end{tabular}}
%     \caption{Ablation on MSR-VTT showing the effect of different loss functions in pretraining. \textbf{No PT.} No multimodal pretraining. \textbf{DAE.} Refers to the denoising autoencoder loss used by UniVL~\cite{luo2020univl}. \textbf{MLM.} Masked Language Modelling Loss. \textbf{FG.} Forward Generation loss. \textbf{BG.} Backward Generation loss. \textbf{WD.} Weight Decay. } 
%     \label{tab:abl-losses}
% \end{table}

\subsubsection{Pretraining Losses} 
\label{sec:abl-losses}
Table~\ref{tab:comps-loss} compares our proposed pretraining loss function to existing losses used in UniVL~\cite{luo2020univl} and CoMVT~\cite{seo2021look}. 
% \arsha{cite} 
We implement these losses with our model architecture for a fair comparison. 
Note that UniVL pretrains both the encoder and the decoder using five different losses whereas CoMVT pretrains only the multimodal encoder.
For CoMVT, we finetune the model with a randomly initialized decoder.
As expected, we first note that all pretraining methods significantly improve captioning performance over training from scratch. We also note that using the UniVL loss and our proposed MV-GPT loss, outperforms CoMVT with large margins. 
% \arsha{We haven't clarified here how we use CoMVT for captioning. We gotta say that we just use the encoder from CoMVT. I think it would also be good to have one line refreshing the losses in UniVL}.
Similarly, if we utilize only the encoder weights of the pretrained MV-GPT, the performance drops significantly.
This indicate the importance of the joint pretraining of the encoder and the decoder.
Finally, compared to UniVL, MV-GPT achieves relative improvements ranging from 5.8\% to 9.5\% across the four evaluation metrics thanks to the use of the future utterances and its bidirectional nature.
Note that UniVL splits a single ASR into partial signals by masking 
% \arsha{you mean by masking right? Or does partial signal mean something else here?}
to use as input and output whereas MV-GPT uses the next utterance as an additional textual supervision and mitigate the temporal mismatch 
%\anurag{Maybe I am mistaken, but this invites a comparison to MIL-NCE~\cite{miech2020end}}
through its bidirectional losses.


Table~\ref{tab:abl-losses} shows the effect of each term in our loss function.
The forward generation (FG) loss already provides strong self-supervision.
When applying the masked language modeling loss on the decoder outputs (MLM-D) instead of the encoder outputs (corresponding non-checked rows), performances are slightly improved thanks to the additional input contextualization provided by the decoder.
% Performance is slightly improved by applying the masked language modeling loss on the decoder outputs (MLM-D) instead of the encoder outputs.
% \arsha{We need to explain this better in Sec. 3.1 and then here we need to provide some reason why we think it helps}.
% \anurag{+1. Also I feel like you need to show a row with MLM-E to substantiate this}
When adopting the full bidrectional loss with the backward generation (BG), the results show significant gains on all metrics.
Additionally, we observe that adding weight decay~\cite{krogh1992simple} brings additional gains and we report our scores in this full setting for the rest of the paper.
%\anurag{Weight decay seems a bit orthogonal to the contribution of this paper. Is it possible to use weight decay everywhere, and mention this as an implementation detail?}


% the following different losses on the YouCook2 dataset.
% \textbf{No PT:} No pretraining (training the model from scratch on YouCook2), \noindent\textbf{DAE:} Denoising auto-encoder. Refers to the generative loss used by UniVL~\cite{luo2020univl}. Given a masked current utterance, we generate the unmasked sentence.  
% \noindent\textbf{FG:} Forward Generation loss. 
% \noindent\textbf{BG:} Backward Generation loss.  
% \noindent\textbf{MLM:} Masked Language Modeling. We test MLM applied in two ways - first applied only on the multimodal encoder outputs (as done in UniVL) and secondly on the decoder outputs.
% \noindent\textbf{WD:} Weight Decay.

% The results show that all pretraining ablations significantly improve model performance compared to training from scratch. We also show a qualitative result in Fig. \ref{fig:youcook_ex}.
% Although DAE pretraining improves performance over training from scratch, FG alone already outperforms DAE in most metrics, confirming our intuition that generating a new unseen utterance is a stronger form of supervision than predicting masked inputs.
% % since most of the output tokens in DAE are already given as inputs providing weaker supervisory signals to the network.
% Our bidirectional generation loss further improves the scores significantly in all metrics.
% Additionally, we observe that applying MLM on the decoder outputs works better than on the multimodal encoder outputs, signalling that the decoder can be used to learn multimodal contexualization of tokens as well as sentence generation.
% % This signifies that our decoder does not only take the role of the sentence generation but also perform the multimodal contextualization within the context inputs.
% Finally, combining all proposed losses achieves the best score, with additional improvements from using weight decay.
% This configuration is used for the rest of our experiments.
% Compared to the DAE loss of~\cite{luo2020univl}, we observe relative improvements ranging from 5.8\% to 9.5\% across the four evaluation metrics. 

% \begin{table}[t]
%     \centering
%     \scalebox{0.73}{
%     \begin{tabular}{lccccc}
%     \toprule
%         Visual Encoder & E2E & B-4 & C & M & R-L \\
%     \midrule 
% S3D (kinetics) & & 17.59 & 1.65 & 22.13 & 42.11 \\% 1254K
% S3D (HowTo100M) & & 18.03 & 1.74 & 22.79 & 43.19 \\ % 1268K
% VIVIT (scratch) & \checkmark &  19.04 & 1.85 & 24.18 & 44.91 \\ % 644K
% VIVIT (kinetics) & &  \\
% VIVIT (kinetics) & \checkmark & 20.08 & 2.00 & 25.33 & 47.03 \\
%     \bottomrule
%     \end{tabular}}
%     \caption{Ablation on YouCook2 with different visual encoder configurations. \textbf{E2E.} End-to-end training in both pretraining and finetuning.}
%     \label{tab:abl-backbone}
% \end{table}


\begin{table}[t]
    \centering
    \scalebox{0.75}{
    \begin{tabular}{@{\hskip 0.8mm}c@{\hskip 1.5mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 0.8mm}}
    \toprule
        Architecture  & Weights from & Trained on & B-4 & C & M & R-L \\
    \midrule 
S3D & S3D \cite{xie2018rethinking} & Kinetics & 18.42 & 1.80 & 23.49 & 44.02 \\% 1254K
S3D & MIL-NCE \cite{miech2020end} & HowTo100M & 19.22 & 1.89 & 24.37 & 45.23 \\ % 1268K
 \hdashline
ViViT & ViViT \cite{arnab2021vivit} & Kinetics & 18.23 & 1.77 & 23.01 & 43.37 \\
ViViT & MV-GPT (Ours)$\dagger$ & HowTo100M & 20.90 & 2.12 & 26.16 & 47.87 \\
    \bottomrule
    \end{tabular}}
    \caption{Ablation on YouCook2 with different visual encoders.
    We pretrain and finetune the other components using our method with a frozen visual encoder.
    $\dagger$ The visual encoder is learned in pretraining and is frozen in finetuning.}
    \label{tab:abl-backbone}
\end{table}


\begin{table}[t]
    \centering
    \scalebox{0.85}{
    \begin{tabular}{cccccc}
    \toprule
        Frozen VE & Frozen MME & B-4 & C & M & R-L \\
    \midrule 
    \multicolumn{6}{c}{\textit{YouCook2}} \\
    \midrule
% VIVIT (Kinetics) & & \\
 &  & \bf20.94 & 2.10 & \bf26.50 & \bf48.38 \\
\checkmark &  & 20.90 & \bf2.12 & 26.16 & 47.87 \\
\checkmark & \checkmark & 18.90 & 1.89 & 23.82 & 44.73 \\
% VIVIT (Kinetics) & Scratch D & 15.50 & 1.37 & 20.28 & 39.94 \\
    \midrule 
    \multicolumn{6}{c}{\textit{MSR-VTT}} \\
    \midrule
 & & \bf48.07 & \bf0.59 & \bf38.12 & \bf64.01 \\
\checkmark &  & 47.64 & 0.56 & 37.56 & 62.85\\
\checkmark & \checkmark & 45.94 & 0.52 & 36.88 & 61.37\\
    \bottomrule
    \end{tabular}}
    \caption{Ablation on YouCook2 and MSR-VTT freezing different modules. \textbf{Frozen MME:} Frozen multimodal encoder, only the decoder is finetuned. \textbf{Frozen VE:} The visual encoder is frozen. 
    \phseo{Add ViViT(scratch) to the appendix.}
    }
    \label{tab:abl-e2e}
\end{table}


% \begin{table}[t]
%     \centering
%     \scalebox{0.7}{
%     \begin{tabular}{lcccccc}
%     \toprule
%         Visual Encoder & E2E PT & E2E FT & B-4 & C & M & R-L \\
%     \midrule 
%     \multicolumn{7}{c}{\textit{YouCook2}} \\
%     \midrule
% S3D (Kinetics) & Frozen VE & Frozen VE & 18.42 & 1.80 & 23.49 & 44.02 \\% 1254K
% S3D (HowTo100M) & Frozen VE & Frozen VE & 19.22 & 1.89 & 24.37 & 45.23 \\ % 1268K
% VIVIT (Scratch) & \checkmark & \checkmark & 19.95 & 2.00 & 25.26 & 46.59 \\ % 644K
% % VIVIT (Kinetics) & & \\
% VIVIT (Kinetics) & \checkmark & Frozen MME & 18.90 & 1.89 & 23.82 & 44.73 \\
% VIVIT (Kinetics) & Frozen VE & Frozen VE & 18.23 & 1.77 & 23.01 & 43.37 \\
% VIVIT (Kinetics) & \checkmark & Frozen VE & 20.90 & 2.12 & 26.16 & 47.87 \\
% \color{red} VIVIT (Kinetics) & \checkmark & Scratch D & 15.50 & 1.37 & 20.28 & 39.94 \\
% VIVIT (Kinetics) & \checkmark & \checkmark & 20.94 & 2.10 & 26.50 & 48.38 \\
%     \midrule 
%     \multicolumn{7}{c}{\textit{MSR-VTT}} \\
%     \midrule
% VIVIT (Kinetics) & \checkmark & Frozen VE & 47.64 & 0.56 & 37.56 & 62.85\\
% VIVIT (Kinetics) & \checkmark & \checkmark & 48.07 & 0.59 & 38.12 & 64.01 \\
%     \bottomrule
%     \end{tabular}}
%     \caption{Ablation on YouCook2 and MSR-VTT with different visual encoders. \textbf{E2E PT:} End-to-end pretraining. \textbf{E2E FT:} End-to-end finetuning. \textbf{Frozen MME:} Frozen multimodal encoder, only the decoder is finetuned. \textbf{Frozen VE:} Only the visual encoder is frozen. A \checkmark indicates all weights are updated during training.}
%     \label{tab:abl-backbone}
% \end{table}



% \begin{table}[t]
%     \centering
%     \scalebox{0.7}{
%     \begin{tabular}{lcccccc}
%     \toprule
%         Visual Encoder & E2E PT & E2E FT & B-4 & C & M & R-L \\
%     \midrule 
%     \multicolumn{7}{c}{\textit{YouCook2}} \\
%     \midrule
% S3D (Kinetics) & Frozen VE & Frozen VE & 17.59 & 1.65 & 22.13 & 42.11 \\% 1254K
% S3D (HowTo100M) & Frozen VE & Frozen VE & 18.03 & 1.74 & 22.79 & 43.19 \\ % 1268K
% VIVIT (Scratch) & \checkmark & \checkmark & 19.04 & 1.85 & 24.18 & 44.91 \\ % 644K
% % VIVIT (Kinetics) & & \\
% VIVIT (Kinetics) & \checkmark & Frozen MME & 18.37 & 1.81 & 23.36 & 44.07 \\
% VIVIT (Kinetics) & Frozen VE & Frozen VE & 17.59 & 1.68 & 21.94 & 41.81 \\
% VIVIT (Kinetics) & \checkmark & Frozen VE & 20.32 & 2.02 & 25.32 & 46.73 \\
% \color{red} VIVIT (Kinetics) & \checkmark & Scratch D & 15.50 & 1.37 & 20.28 & 39.94 \\
% VIVIT (Kinetics) & \checkmark & \checkmark & 20.94 & 2.10 & 26.50 & 48.38 \\
%     \midrule 
%     \multicolumn{7}{c}{\textit{MSR-VTT}} \\
%     \midrule
% VIVIT (Kinetics) & \checkmark & Frozen VE & 48.19 & 0.55 & 37.41 & 62.73\\
% VIVIT (Kinetics) & \checkmark & \checkmark & 48.07 & 0.59 & 38.12 & 64.01 \\
%     \bottomrule
%     \end{tabular}}
%     \caption{Ablation on YouCook2 and MSR-VTT with different visual encoders. \textbf{E2E PT:} End-to-end pretraining. \textbf{E2E FT:} End-to-end finetuning. \textbf{Frozen MME:} Frozen multimodal encoder, only the decoder is finetuned. \textbf{Frozen VE:} Only the visual encoder is frozen. A \checkmark indicates all weights are updated during training.}
%     \label{tab:abl-backbone}
% \end{table}

% \begin{table}[t]
%     \centering
%     \scalebox{0.63}{
%     \begin{tabular}{lcccccc}
%     \toprule
%         Visual Encoder & E2E PT & E2E FT & B-4 & C & M & R-L \\
%     \midrule 
% VIVIT (kinetics) & \checkmark & No vis enc & 48.19 & 0.55 & 37.41 & 62.73\\
% VIVIT (kinetics) & \checkmark & \checkmark & 48.07 & 0.59 & 38.12 & 64.01 \\
%     \bottomrule
%     \end{tabular}}
%     \caption{Ablation on MSR-VTT with different visual encoder configurations.}
%     \label{tab:abl-backbone-msrvtt}
% \end{table}

% \begin{table}[t]
%     \centering
%     \scalebox{0.63}{
%     \begin{tabular}{lcccccc}
%     \toprule
%         Visual Encoder & E2E PT & E2E FT & B-4 & C & M & R-L \\
%     \midrule 
% S3D (kinetics) & & & 46.56 & 0.54 & 36.87 & 62.56 \\
% S3D (HowTo100M) & & & 44.45 & 48.12 & 35.66 & 60.75 \\ % 1268K
% VIVIT (scratch) & \checkmark & \checkmark & 45.99 & 0.54 & 36.47 & 62.44 \\ % 644K
% VIVIT (kinetics) & & \\
% VIVIT (kinetics) & \checkmark & Dec only & 45.94 & 0.52 & 36.88 & 61.37 \\
% VIVIT (kinetics) & \checkmark & No vis enc & 48.19 & 0.55 & 37.41 & 62.73\\
% VIVIT (kinetics) & \checkmark & \checkmark & 48.07 & 0.59 & 38.12 & 64.01 \\
%     \bottomrule
%     \end{tabular}}
%     \caption{Ablation on MSR-VTT with different visual encoder configurations.}
%     \label{tab:abl-backbone-msrvtt}
% \end{table}

\subsubsection{Visual Encoder and End-to-end Training} 
In Table~\ref{tab:abl-backbone}, we first compare the ViViT~\cite{arnab2021vivit} encoder to commonly used S3D features~\cite{xie2018rethinking}.
When both encoders are trained on Kinetics and fixed for multimodal pretraining and finetuning, they show comparable scores despite the large complexity of S3D due to the high frame rate required (30 fps vs. 1 fps for ViViT).
Using HowTo100M to train a visual encoder, we observe large gains with both architectures as expected given the similarity in domains -- HowTo100M and YouCook2 are both instructional video datasets.
However, we observe larger gains with ViViT when the visual encoder is optimized for  generative losses within our framework and jointly trained with the other components thanks to its low complexity.
These results show the benefits of end-to-end pretraining.

% In Table~\ref{tab:abl-backbone}, we compare the ViViT~\cite{arnab2021vivit} encoder to commonly used S3D features~\cite{xie2018rethinking}.
% S3D features trained on HowTo100M as in \cite{miech2020end} outperform those trained on Kinetics (as expected given the similarity in domain - HowTo100M and YouCook2 are both instructional video datasets). In both cases the S3D features are frozen, because end-to-end training with S3D features is computationally infeasible on long videos given the high frame rate of consecutive frames required (30 fps). Using a ViViT encoder trained from scratch leads to improved results, despite the coarse frame sampling and the fact that there is no initialisation \eg\ from Kinetics. This is further improved by initialising the visual encoder with weights from a Kinetics-400 trained model.

We further investigate the importance of end-to-end training in Table~\ref{tab:abl-e2e}.
We freeze some components such as the visual encoder while finetuning the other components, which is the setting commonly adopted in all previous approaches for multimodal video pretraining~\cite{luo2020univl,li2020hero, tang2021decembert,huang2020multimodal}.
When we freeze the visual encoder, we get similar performance on YouCook2, but the performance drop on MSR-VTT -- this is because end-to-end training allows our model to better adapt to the target domain (which is different for MSR-VTT as it does not consist of instructional videos).
If we freeze the entire multimodal encoder and finetune the decoder only, the performance drops further on both datasets.
% \anurag{We never say ``performances''}


% If we freeze only the visual encoder, we get similar performance on YouCook2, but performance drops on MSR-VTT -- this is because end-to-end training allows our model to better adapt to the target domain (which is different for MSR-VTT as it does not consist of instructional videos). 
% We also note that finetuning the decoder only gives worse performance than finetuning the entire model.
% \red{
% Finally, if we use the pretrained weights to initialize only the multimodal encoder and train the decoder from scratch during the finetuning\footnote{We still initialize the decoder using pretrained GPT-2 weights on the text dataset.}, the performance drops significantly. This indicates the importance of the joint pretraining of both encoder and decoder for captioning, and shows the limitation of the encoder-only pretraining techniques.
% }


\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/scale_eval.png}
    \caption{Performance changes in four captioning metrics with varying pretraining dataset sizes on YouCook2 for video captioning. }
    \label{fig:scale}
\end{figure}

\subsubsection{Dataset Sizes and Multimodality}
Figure~\ref{fig:scale} reports performance against dataset size. 
All four metrics show improvement (almost linear) when the dataset size is doubled. 
This signifies the potential gains from collecting more unlabeled videos for pretraining. 
% \arsha{We need something to say here. Hence we would expect further performance gains with more data? Performance is not yet saturated?}
% \anurag{Yes, but this could also suggest that you need a lot more data to get a small improvement. So don't know if its worth mentioning}
% \phseo{Should we move this to the supplementary?}


\begin{table}[t]
    \centering
    \scalebox{0.85}{
    \begin{tabular}{@{\hskip 0.8mm}l@{\hskip 1mm}c@{\hskip 2.5mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 0.8mm}}
    \toprule
        Method & PT parts & Inputs & B-4 & C & M & R-L \\
    \midrule 
        Bi-LSTM~\cite{zhou2018towards} & -- & V & 0.87 & -- & 8.15 & -- \\
        EMT~\cite{zhou2018end} & -- & V & 4.38 & 0.38 & 11.55 & 27.44 \\
        VideoBERT~\cite{sun2019videobert} & E & V & 4.04 & 0.49 & 11.01 & 27.50 \\
        CBT~\cite{sun2019learning} & E & V & 5.12 & 0.64 & 12.97 & 30.44 \\
        ActBERT~\cite{zhu2020actbert} & E & V & 5.41 & 0.65 & 13.30 & 30.56 \\
        VideoAsMT~\cite{korbar2020video} & E & V & 5.30 & -- & 13.40 & --\\
        MART~\cite{lei2020mart} & -- & V & 8.00 & 0.36 & 15.90 & --\\
        AT~\cite{hessel2019case} & -- & T & 8.55 & 1.06 & 16.93 & 35.54 \\ 
        \hdashline
        DPC~\cite{shi2019dense} & -- & V+T & 2.76 & -- & 18.08 & -- \\
        AT+Video~\cite{hessel2019case} & -- & V+T & 9.01 & 1.12 & 17.77 & 36.65 \\ 
        % \hdashline
        DECEMBERT~\cite{tang2021decembert} & E & V+T & 11.92 & 0.58 & 20.01 & 40.22 \\
        M-MASS~\cite{huang2020multimodal} & E+D & V+T & 12.04 & 1.23 & 18.32 & 39.03 \\
        UniVL~\cite{luo2020univl} & E+D & V+T & 17.35 & 1.81 & 22.35 & 46.52 \\ 
        \hdashline
        MV-GPT (Ours) & E+D & V & 16.71 & 1.53 & 21.43 & 41.56 \\ % 1054K
        % MV-GPT (Ours)$\dagger$ & T* & 14.26 & 1.18 & 17.44 & 34.99 \\
        MV-GPT (Ours) & E+D & T & 15.49 & 1.40 & 19.71 &     37.82 \\ 
        \bf MV-GPT (Ours) & \bf E+D & \bf V+T & \bf 20.94 & \bf2.10 & \bf 26.50 & \bf 48.38 \\ \midrule
        Human~\cite{hessel2019case} & -- & V+T & 15.20 & 3.80 & 25.90 & 45.10 \\
    \bottomrule
    \end{tabular}}
    \caption{Comparison to SOTA on YouCook2 for video captioning. 
    }
    \label{tab:sota-youcook}
\end{table}

% \subsubsection{Multimodal vs Single Modality}
In Table~\ref{tab:sota-youcook}, we show results with text only and visual only inputs (we just feed the \texttt{CLS} token for the omitted modality). It is clear that both modalities are complementary and performance is best when combining both.
% We note that our vision-only model performs better than the text-only model -- however this is because we were unable to obtain ASR transcripts for all the videos in the YouCook2 validation set. We conjecture that all our results could be further improved if we had access to the ASR for all videos, as used in other works.
% We conjecture that our visual encoder is tuned end-to-end and the model relies more on the visual inputs.

\begin{table}[t]
    \centering
    \scalebox{0.85}{
    % \resizebox{0.99\linewidth}{!}{
    \begin{tabular}{@{\hskip 0.8mm}l@{\hskip 1mm}c@{\hskip 2.5mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 0.8mm}}
        \toprule
        Method & PT parts & Inputs&  B-1 & C & M & R-L \\
        \midrule
        M-MASS~\cite{huang2020multimodal} & E+D & V+T & 22.37 & 0.82 & 11.00 & 31.40\\ 
        \bf MV-GPT (Ours) &E+D & V+T & \bf 37.89 & \bf 1.04 & \bf 26.75 & \bf 34.76 \\ 
        \midrule
        Human~\cite{huang2020multimodal} & 43.34 & 1.26 & 33.56 & 41.88 \\ 
        \bottomrule
    \end{tabular}}
    \caption{Comparison to SOTA on ViTT for video captioning.}
    \label{tab:sota-vitt}
\end{table}

\begin{table}[t]
    \centering
    \scalebox{0.85}{
    % \resizebox{0.99\linewidth}{!}{
    \begin{tabular}{@{\hskip 0.8mm}l@{\hskip 1mm}c@{\hskip 2.5mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 3mm}c@{\hskip 0.8mm}}
    \toprule
        Method & PT parts & Inputs & B-4 & C & M & R-L \\
        \midrule 
        MARN~\cite{pei2019memory} & -- & V & 40.40 & 0.47 & 28.10 & 60.70 \\
        SibNet~\cite{liu2020sibnet} & -- & V & 40.90 & 0.48 & 27.50 & 60.20 \\
        OA-BTG~\cite{zhang2019object} & -- & V & 41.40 & 0.47 & 28.20 & -- \\
        GRU-EVE~\cite{aafaq2019spatio} & -- & V & 38.30 & 0.48 & 28.40 & 60.70 \\
        MGSA~\cite{chen2019motion} & -- & V & 42.40 & 0.48 & 27.60 &  -- \\
        POS+CG~\cite{wang2019controllable} & -- & V & 42.00 & 0.49 & 28.20 & 61.60 \\
        POS+VCT~\cite{hou2019joint} & -- & V & 42.30 & 0.49 & 29.70 & 62.80 \\
        SAM-SS~\cite{chen2020semantics} & -- & V & 43.80 & 0.51 & 28.90 & 62.40 \\
        ORG-TRL~\cite{zhang2020object} & -- & V & 43.60 & 0.51 & 28.80 & 62.80 \\
        VNS-GRU~\cite{chen2020delving} & -- & V & 45.30 & 0.53 & 29.90 & 63.40\\ \hdashline
        DECEMBERT~\cite{tang2021decembert} & E & V & 45.20 & 0.52 & 29.70 & \bf 64.70 \\ 
        UniVL~\cite{luo2020univl} & E+D & V+T & 41.79 & 0.50 & 28.94 & 60.78 \\
        \hdashline
        \bf MV-GPT (Ours) & E+D & V+T & \bf 48.07 & \bf 0.59 & \bf 38.12 & 64.01 \\ 
        \bottomrule
    \end{tabular}}
    \caption{Comparison to SOTA on MSR-VTT for video captioning. $\dagger$ Models pretrained on HowTo100M.}
    \label{tab:sota-msr}
\end{table}

\begin{table}[t]
    \centering
    \scalebox{0.85}{
    % \resizebox{0.99\linewidth}{!}{
    \begin{tabular}{@{\hskip 0.8mm}lcccc@{\hskip 0.8mm}}
    \toprule
        Method & B-4 & M \\
        \midrule 
        DCEV~\cite{krishna2017dense} & 1.60 & 8.88 \\
        DVC~\cite{li2018jointly} & 1.71 & 9.31 \\
        Bi-SST~\cite{wang2018bidirectional}& -- & 10.89 \\
        HACA~\cite{wang2018watch} & 2.71 & 11.16 \\
        MWSDEC~\cite{rahman2019watch} & 1.46 & 7.23 \\
        MDVC~\cite{iashin2020multi} & 1.46 & 7.23 \\
        BMT~\cite{iashin2020better} & 1.99 & 10.90 \\\hdashline
        \bf MV-GPT (Ours) & \bf 6.84 & \bf 12.31 \\ 
        \bottomrule
    \end{tabular}}
    \caption{
    Comparison to SOTA on ActivityNet-Captions for video captioning with ground-truth action proposals.}
    \label{tab:sota-activitynet}
\end{table}



\begin{figure*}
    \centering
    \scalebox{0.85}{
        \begin{tabular}{@{\hskip 0.8mm}c@{\hskip 7mm}c@{\hskip 0.8mm}}

            % Example1: WYAFPvlDB_A-005
            \begin{tabular}{@{\hskip 0.8mm}p{9cm}@{\hskip 2mm}p{4.3cm}@{\hskip 0.8mm}}
                \centering
                \adjincludegraphics[valign=c,width=0.48\linewidth]{figures/3_1.jpeg}~
                \adjincludegraphics[valign=c,width=0.48\linewidth]{figures/3_2.jpeg}
                &\parbox[c]{1\linewidth}{\textbf{Transcript}: This makes a really good source. So about twenty five spice you like it. That's about 4 teaspoons where take your tuna.}
                
            \end{tabular}
            & 
            \bgroup
            
            \begin{tabular}{@{\hskip 0mm}l@{\hskip 0.8mm}}
                \raggedright \textbf{Generated captions}  \tabularnewline[1.2mm]
                \raggedright ~\colorbox[RGB]{220,230,242}{GT:} pour in spicy sauce \tabularnewline[1mm]
                \raggedright ~\colorbox[RGB]{242,220,219}{No-PT:} pour some sauce over the pasta \tabularnewline[1mm]
                \raggedright ~\colorbox[RGB]{242,220,219}{UniVL:} add mayo to the bowl \tabularnewline[1mm]
                \raggedright ~\colorbox[RGB]{235,241,222}{MV-GPT:} add sriracha to the bowl \tabularnewline
            \end{tabular}
            \egroup \\ 
    
        \end{tabular}
    }
    \caption{Qualitative example on YouCook2. \colorbox[RGB]{220,230,242}{GT:} Ground-truth caption. \colorbox[RGB]{242,220,219}{No-PT:} No multimodal pretraining on HowTo100M. \colorbox[RGB]{242,220,219}{UniVL:} Previous pretrained SOTA model. \colorbox[RGB]{235,241,222}{MV-GPT:} Our pretrained model. Despite the ASR error \textit{sauce}$\rightarrow$\textit{source}, our model is able to generate the precise name of the sauce from the input frames.
    In contrast, UniVL misrecognizes the sauce as 'mayo' and No-PT erroneously generates the word 'pasta'.
    %, unlike the model without pretraining which erroneously generates the word `pasta'.
    }
    \label{fig:youcook_ex}
\end{figure*}

\subsubsection{Comparisons to the State of the Art} 
%\noindent\textbf{Video Captioning:} 
Table~\ref{tab:sota-youcook} compares our method to state of the art works on YouCook2. 
Our method outperforms all prior work, including M-MASS and UniVL which also both pretrain on HowTo100M. % \anurag{This makes it sound like M-MASS and UniVL are the only comparable works in the table}. 
On ViTT (Table~\ref{tab:sota-vitt}), the gaps are even larger, with our model advancing the state-of-the-art by 15\% (absolute) compared to M-MASS in the BLEU-1 and Meteor scores. %\anurag{Why is the gap so much larger on this dataset? Because of the end-to-end training of the visual encoder?}
%achieveing the state of the art results by ~15\% absolute improvement over M-MASS in the BLEU-1 and Meteor scores.

Despite the domain gap between instructional videos in the pretraining dataset and general online videos in MSR-VTT, our model outperforms all existing work in most of the metrics as shown in Table~\ref{tab:sota-msr}.
% For a fair comparison, we obtain the scores of UniVL on MSR-VTT using the author's code\footnote{\url{https://github.com/microsoft/UniVL}}. 
Although they also use HowTo100M for pretraining, our method achieves relative improvements of over 31\% thanks to our end-to-end training. %\anurag{of the visual encoder?}.
Similarly, Table~\ref{tab:sota-activitynet} shows that our pretraining method achieves the state-of-the-art performances on ActivityNet-Captions despite the significant domain gap.
We show qualitative results in Figure~\ref{fig:youcook_ex}.

% {
% \color{red}
% \subsubsection{Efficient Transfer to Captioning}
% \phseo{Test the captioning performances with zero-shot / few-shot settings.
% Add the results to Table 3 and 5.
% If the results present good performances, it can be because the model already produces content-related captions but their styles are different (pragmatic vs. narrative). }
% }

	
\begin{table}[t]
    \centering
    \scalebox{0.8}{
    \begin{tabular}{@{\hskip 0.8mm}l@{\hskip 1mm}c@{\hskip 0mm}c@{\hskip 2mm}c@{\hskip 0.8mm}}
    \toprule
        Method & Pretrained on & MSRVTT-QA & ActivityNet-QA \\
    \midrule 
        E-SA~\cite{yu2019activitynet} & -- & 29.3 & 31.8\\
        SSML~\cite{amrani2020noise} & HowTo100M~\cite{miech2019howto100m} & 35.1 & --\\
        MAR-VQA~\cite{zhuang2020multichannel} & -- & -- & 34.6\\
        ClipBERT~\cite{lei2021less} & COCO~\cite{chen2015microsoft}+VG~\cite{krishna2017visual} & 37.4 & --\\
        DECEMBERT~\cite{tang2021decembert} & HowTo100M~\cite{miech2019howto100m} & 37.4 & -- \\
        CoMVT~\cite{seo2021look} & HowTo100M~\cite{miech2019howto100m} & 39.5 & 38.8\\
        VQA-T~\cite{yang2020just} &  HowToVQA~\cite{yang2020just} & 41.5 & 38.9 \\ \hdashline
        \bf MV-GPT (Ours) & \textbf{HowTo100M}~\cite{miech2019howto100m} & \bf 41.7 & \bf 39.1\\% 25328956-8
    \bottomrule
    \end{tabular}}
    \caption{Comparison to SOTA on MSRVTT-QA and ActivityNet-QA for video question answering. Our method is comparable to other works, even those designed specifically for the task of VideoQA.}
    \label{tab:vqa}
\end{table}
\subsubsection{MV-GPT as a Multimodal Encoder}
Although MV-GPT is a generative model, we also test it as a multimodal video encoder, specifically for the task of video question answering (VideoQA) on MSRVTT-QA and ActivityNet-QA (Table~\ref{tab:vqa}). 
% \arsha{It's not clear exactly how this is trained, we don't have the decoder at all here right? Or do we train with the generative losses as well for retrieval?}
% We test our model for VideoQA on MSRVTT-QA and ActivityNet-QA and Table~\ref{tab:vqa} compares our model to the previous state of the art methods.
Even though MV-GPT is not designed for this particular task, our model slightly outperforms the previous state-of-the-art VQA-T~\cite{yang2020just} (which is specifically designed for VideoQA) on both datasets.
% Although MV-GPT is not designed for this particular task, our model slightly outperforms on both benchmarks the best existing model VQA-T, which pretrains specifically targeting VideoQA only.
% \phseo{add details to the supplementary}


\begin{table}[t]
    \centering
    \scalebox{0.85}{
    \begin{tabular}{@{\hskip 0.8mm}lcccc@{\hskip 0.8mm}}
    \toprule
        Method & R@1 & R@5 & R@10 & MdR \\
    \midrule 
        UniVL~\cite{luo2020univl} & 21.2 & 49.6 & 63.1 & 6 \\
        MMT~\cite{gabeur2020Learning} & 26.6 & 57.1 & 69.6 & 4\\
        AVLnet~\cite{rouditchenko2021avlnet} & 27.1 & 55.6 & 66.6 & 4\\
        SSB~\cite{patrick2021supportset} & 30.1 & 58.5 & 69.3 & \bf3 \\
        HiT~\cite{liu2021hit} & 30.7 & 60.9 & 73.2 & -- \\ \hdashline
        % \bf MV-GPT (Ours) & \bf 34.3 & \bf 62.7 & \bf 74.3 \\
        \bf MV-GPT w/o ASR (Ours) & \bf 33.6 & \bf 61.2 & \bf 73.6 & \bf3 \\
        \bf MV-GPT w/ ASR (Ours) & \bf 37.3 & \bf 65.5 & \bf 75.1 & \bf2\\
    \bottomrule
    \end{tabular}}
    \caption{Comparison to SOTA on MSR-VTT for video retrieval.
    We compare models pretrained on HowTo100M. \textbf{R@$\boldsymbol{k}$}: Recall at $k$. \textbf{MdR}: Median rank. 
    %\phseo{The numbers for our model should be updated.}
    }
    \label{tab:retrieval_msr}
\end{table}

Similarly, we also evaluate our multimodal encoder for the video retrieval task on MSR-VTT. 
We pretrain our model with an additional NCE loss and a textual encoder to enforce a joint embedding space between multimodal videos and text queries. 
For detailed settings, refer to the supplementary.
Table~\ref{tab:retrieval_msr} clearly shows that MV-GPT outperforms the existing models in the fair configuration.
Moreover, feeding ASR to our multimodal encoder further improves the performance.

% \arsha{I think potentially reviewers might ask for performance without HowTo100M pretraining, to see how much gain comes from pretraining and how much from our model architecture}.


\subsubsection{MV-GPT as Cross-modal Pretraining}
Finally, Table~\ref{tab:kinetics} demonstrates that MV-GPT is an effective pretraining strategy for the visual encoder.
High-capacity transformer models like ViViT are challenging to train from scratch, and overfit easily as shown in the first row.
However, ViVIT initialised from an MV-GPT visual encoder trained from scratch performs substantially better, obtaining absolute improvements of 24\% on Kinetics-400 (a standard video classification benchmark).
This figure approaches the performance of ViViT initalized with ImageNet-21K pretraining, as done by the original authors~\cite{arnab2021vivit} (note that ImageNet-21K was created with high manual annotation cost, while we used no labels at all during pretraining).
Finally, initialising the MV-GPT visual encoder with these same ImageNet-21K weights, and then pretraining the MV-GPT visual encoder weights on HowTo100M achieves the best results, improving upon the initialisation of~\cite{arnab2021vivit} by 1.5\% and 1.8\% on Kinetics-400 and Kinetics-600 respectively, which is the current state of the art on this dataset with this model.
% Table~\ref{tab:kinetics} therefore demonstrates that our pretraining process learns strong visual representations from unlabelled videos.

\iffalse
    Finally, Table~\ref{tab:kinetics} presents the of the same ViViT architecture on Kinetics~\cite{kay2017kinetics}, \anurag{the largest dataset for action classification}, with different initializations.
    When ViViT is initialized the visual encoder weights of \model pretrained from scratch (ViViT+MV-GPT), this already gives more than 20\% absolute improvements in both Kinetics 400 and 600 compared to ViViT-scratch, which is trained from scratch.
    Note that ViViT+MV-GPT does not use any labeled datasets.
    Even when we use an additional labeled dataset, \cs{check refernce} ImageNet21k~\cite{deng2009imagenet}, to initialize ViViT as in \cite{arnab2021vivit}, we find that our pretraining still improves the quality of the visual representation by more than 1\% of accuracy.
    These results clearly indicate that our pretraining process learns strong visual representations from unlabeled videos.
    \anurag{Maybe emphasise that - 
    	High capacity models like ViViT overfit easily, so very challenging to train from scratch.
    	MV-GPT pre-training allows one to train ViViT from scratch, and finetune on Kinetics.
    	The result of this approaches ViViT initialised from an ImageNet-21K pretrained model as used by~\cite{arnab2021vivit}.
    	Best results are obtained if the ViViT part of MV-GPT is initialised from an ImageNet-21K model, trained in a self-supervised fashion, and then finetuned on Kinetics.
    }
    \todo{distinguish between name of model, and name of pretraining strategy}

\begin{table}[t]
    \centering
    \scalebox{0.73}{
    \begin{tabular}{@{\hskip 0.8mm}lcc@{\hskip 0.8mm}}
    \toprule
        ViViT initialization & Kinetics-400 & Kinetics-600 \\ % & MSVD-QA \\
    \midrule 
         ViViT-scratch & 47.46 & ~55.xx \\  %(21919230, 52), (25255668, 19)
         ViViT+MV-GPT$\dagger$ & 71.88 & 75.69 \\ % (25218971, 1), (25219017, 1)
         ViViT+ImageNet21k & 76.93 & 79.74 \\     % (21356628, 13), (25219017, 4)
         ViViT+ImageNet21k+MV-GPT$\dagger$ & 78.73 & 81.10 \\  % (25218971, 2) (25219017, 2)
        % None & & 41.5 \\ % & 46.3 \\
        % Ours \\
    \bottomrule
    \end{tabular}}
    \caption{Action classification results on Kinetics with different ViViT initialization. $\dagger$\model refers to initialization from our visual encoder weights in \model pretrained on HowTo100M with \textit{no action classification} labels.}
    \label{tab:kinetics}
\end{table}
\fi

\begin{table}[t]
    \centering
    \scalebox{0.85}{
    \begin{tabular}{@{\hskip 0.8mm}lcc@{\hskip 0.8mm}}
    \toprule
        ViViT initialization & Kinetics-400 & Kinetics-600 \\ % & MSVD-QA \\
    \midrule 
         Scratch & 50.14 & 55.47 \\  %(21919230, 52), (25255668, 19)
         MV-GPT$\dagger$ & 74.20 & 77.10 \\ % (25218971, 1), (25219017, 1)
         \hdashline
         ImageNet21k~\cite{arnab2021vivit} & 78.90 & 80.62 \\     % (21356628, 13), (25219017, 4)
         ImageNet21k + MV-GPT$\dagger$ & 80.40 & 82.42 \\  % (25218971, 2) (25219017, 2)
        % None & & 41.5 \\ % & 46.3 \\
        % Ours \\
    \bottomrule
    \end{tabular}}
    \caption{Action classification results on Kinetics with different ViViT initializations. MV-GPT$\dagger$ refers to a model initalised with our MV-GPT pretraining on HowTo100M with \textit{no manually annotated} labels.}
    \label{tab:kinetics}
\end{table}

